Label Smarter, Not Harder: CleverLabel for Faster Annotation of Ambiguous Image Classification with Higher Quality

High-quality data is crucial for the success of machine learning, but labeling large datasets is often a time-consuming and costly process. While semi-supervised learning can help mitigate the need for labeled data, label quality remains an open issue due to ambiguity and disagreement among annotators. Thus, we use proposal-guided annotations as one option which leads to more consistency between annotators. However, proposing a label increases the probability of the annotators deciding in favor of this specific label. This introduces a bias which we can simulate and remove. We propose a new method CleverLabel for Cost-effective LabEling using Validated proposal-guidEd annotations and Repaired LABELs. CleverLabel can reduce labeling costs by up to 30.0%, while achieving a relative improvement in Kullback-Leibler divergence of up to 29.8% compared to the previous state-of-the-art on a multi-domain real-world image classification benchmark. CleverLabel offers a novel solution to the challenge of efficiently labeling large datasets while also improving the label quality.

==> CleverLabel Submission PKDD_arXiv/images.tex <==
\graphicspath{{images/}}

\usepackage{caption}
\usepackage{subcaption}

\newcommand{\pic}[3]{
	\begin{figure}[tb] 
		\centering
		\includegraphics[width=#3\linewidth]{#1}
		\caption{#2}
		\label{fig:#1}
	\end{figure}
}

\newcommand{\picLarge}[3]{
	\begin{figure}[tb] 
  \begin{subfigure}[c]{0.98\linewidth}	
			\centering	
			\includegraphics[width=0.9\textwidth]{#1-legend}
		\end{subfigure}
  \begin{subfigure}[c]{0.98\linewidth}	
			\centering	
			\includegraphics[width=#3\textwidth]{#1}
   \label{fig:#1}
		\end{subfigure}
  \caption{#2}
	\end{figure*}
}

\newcommand{\picTwoLarge}[4]{
	\begin{figure*}[tb]
		\centering
        \begin{subfigure}[c]{0.95\linewidth}	
			\centering	
			\includegraphics[width=0.9\textwidth]{#1-legend}
		\end{subfigure}
		\begin{subfigure}[c]{0.45\linewidth}
			\centering		
			\includegraphics[width=0.9\textwidth]{#1-0}
			\subcaption{#2}	
			\label{fig:#1-0}	
		\end{subfigure}
		\begin{subfigure}[c]{0.45\linewidth}	
			\centering	
			\includegraphics[width=0.9\textwidth]{#1-1}
			\subcaption{#3}
			\label{fig:#1-1}	
		\end{subfigure}
		\caption{#4}
		\label{fig:#1}
	\end{figure*}
}


\newcommand{\picTwo}[4]{
	\begin{figure*}[tb]
		\centering
		\begin{subfigure}[c]{0.45\linewidth}
			\centering		
			\includegraphics[width=0.9\linewidth]{#1-0}
			\subcaption{#2}	
			\label{fig:#1-0}	
		\end{subfigure}
		\begin{subfigure}[c]{0.45\linewidth}	
			\centering	
			\includegraphics[width=0.9\linewidth]{#1-1}
			\subcaption{#3}
			\label{fig:#1-1}	
		\end{subfigure}
		\caption{#4}
		\label{fig:#1}
	\end{figure*}
}

\newcommand{\picTwoVertical}[4]{
	\begin{figure}[tb]
		\centering
		\begin{subfigure}[c]{0.9\linewidth}
			\centering		
			\includegraphics[width=0.9\linewidth]{#1-0}
			\subcaption{#2}	
			\label{fig:#1-0}	
		\end{subfigure}
		\begin{subfigure}[c]{0.9\linewidth}	
			\centering	
			\includegraphics[width=0.9\linewidth]{#1-1}
			\subcaption{#3}
			\label{fig:#1-1}	
		\end{subfigure}
		\caption{#4}
		\label{fig:#1}
	\end{figure}
}


\newcommand{\picThree}[5]{
	\begin{figure*}[tb]
		\centering
		\begin{subfigure}[c]{0.325\linewidth}
			\centering		
			\includegraphics[width=0.9\textwidth]{#1-0}
			\subcaption{#2}	
				\label{fig:#1-0}	
		\end{subfigure}
		\begin{subfigure}[c]{0.325\linewidth}	
			\centering	
			\includegraphics[width=0.9\textwidth]{#1-1}
			\subcaption{#3}	
				\label{fig:#1-1}	
		\end{subfigure}
		\begin{subfigure}[c]{0.325\linewidth}	
			\centering	
			\includegraphics[width=0.9\textwidth]{#1-2}
			\subcaption{#4}	
				\label{fig:#1-2}	
		\end{subfigure}
	
		\caption{#5}
		\label{fig:#1}
	\end{figure*}
}

==> CleverLabel Submission PKDD_arXiv/tables.tex <==
\newcommand{\tbldatasetOffsets}{
\begin{table}[tb]
	\caption{
		Used offsets ($\delta$) for proposal  acceptance
	}
	\label{tbl:datasetOffsets}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{p{2.2cm} p{2.2cm} p{2.2cm} p{2.2cm} p{2.2cm} p{2.2cm}}
          
          \toprule           
dataset  & Benthic &  CIFAR10H & MiceBone & Pig & Plankton  \\
 \midrule
User Study & N/A & 9.73\% &  36.36\% & N/A &  57.84\%  \\
Calculated & 40.17\% & 0.00\% & 41.03\% & 25.72\% & 64.81\% \\

\midrule
dataset  &  QualityMRI & Synthethic &  Treeversity\#1 & Treeversity\#6 & Turkey \\
 \midrule
User Study & N/A & N/A & N/A & N/A &  21.64\% \\
Calculated  & 0.00\% & 26.08\% & 26.08\% & 20.67\% & 14.17\% 
			
		\end{tabular}
	}
		
\end{table}
}

\newcommand{\tblSPAResults}{
\begin{table}[tb]
	\caption{
		Comparison of investigated methods for the proposal acceptance, 
        results within a one percent boundary of the best results are marked bold
		$^\dagger$ datasets used only for validation, 
	}
	\label{tbl:SPAComparison}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{p{3.8cm} p{2.2cm} p{2.2cm} p{2.2cm} p{2.2cm}}
                     
 $SOD$ in [\%]  & CIFAR10H $^\dagger$ & MiceBone $^\dagger$ &  Plankton & Turkey \\
 \midrule
ACCEPT+GT (Ours) & \textbf{1.97 $\pm$ 0.06} & \textbf{2.57 $\pm$ 0.16} & \textbf{3.62 $\pm$ 0.05} & \textbf{4.77 $\pm$ 0.13} \\
 ACCEPT+LIKELY & \textbf{1.20 $\pm$ 0.25} & 7.88 $\pm$ 0.06 & 5.50 $\pm$ 0.15 & 7.21  $\pm$ 0.32\\    
2*ACCEPT+GT & 2.79 $\pm$ 0.22 & \textbf{3.38 $\pm$ 0.26} & \textbf{3.25 $\pm$ 0.13} & \textbf{3.78  $\pm$ 0.28} \\
 2*ACCEPT+RANDOM & 3.03 $\pm$ 0.11 & 4.76 $\pm$ 0.11 & \textbf{4.00 $\pm$ 0.31} & \textbf{4.64  $\pm$ 0.28}\\
 RANDOM & 86.37 $\pm$ 0.13 & 50.92 $\pm$ 0.64  & 81.51 $\pm$ 0.18 & 54.83  $\pm$ 0.93\\
 GT & 5.00 $\pm$ 0.03 & 10.34  $\pm$ 0.19 & 10.59 $\pm$ 0.11 & 5.69  $\pm$ 0.30\\
 LIKELY & 4.08 $\pm$ 0.00 & 16.41 $\pm$ 0.00 &  11.85 $\pm$ 0.00 & 11.47  $\pm$ 0.00 
 \end{tabular}
	}
		
\end{table}
}

\newcommand{\tblSimulatedSPAReal}{
\begin{table}[tb]
	\caption{
		Simulation of SPA on Real data, full results for visualized median aggregation in \autoref{fig:simulated-1}
	}
 \centering
	\label{tbl:SimulatedSPAReal}
		\begin{tabular}{l c c c c c c c c c c c c c c c c}
			\toprule
			

                     
 dataset & method & 1 & 3 & 5 & 12 \\
 \midrule
CIFAR10H & GT & 0.71 & 0.25 & 0.21 & 0.13 \\
CIFAR10H & GT+CB & 0.42 & 0.11 & 0.11 & 0.07 \\
CIFAR10H & SPA & 0.81 & 0.53 & 0.37 & 0.30 \\
CIFAR10H & Only BC & 0.81 & 0.53 & 0.37 & 0.30 \\
CIFAR10H & Only CB & 0.42 & 0.34 & 0.28 & 0.20 \\
CIFAR10H & \spaplus (+ GT $\delta$) & 0.47 & 0.26 & 0.20 & 0.16 \\
CIFAR10H & \spaplus & 0.47 & 0.26 & 0.19 & 0.16 \\
Turkey & GT & 1.37 & 0.51 & 0.27 & 0.11 \\
Turkey & GT+CB & 0.35 & 0.14 & 0.08 & 0.04 \\
Turkey & SPA & 2.64 & 1.87 & 0.66 & 0.22 \\
Turkey & Only BC & 2.64 & 1.86 & 0.65 & 0.22 \\
Turkey & Only CB & 0.49 & 0.47 & 0.38 & 0.15 \\
Turkey & \spaplus (+ GT $\delta$) & 0.77 & 0.61 & 0.25 & 0.08 \\
Turkey & \spaplus & 0.77 & 0.61 & 0.26 & 0.08 \\
MiceBone & GT & 2.36 & 0.83 & 0.51 & 0.23 \\
MiceBone & GT+CB & 0.48 & 0.17 & 0.12 & 0.06 \\
MiceBone & SPA & 2.58 & 2.36 & 1.08 & 0.57 \\
MiceBone & Only BC & 2.58 & 2.36 & 1.17 & 0.61 \\
MiceBone & Only CB & 0.31 & 0.32 & 0.29 & 0.21 \\
MiceBone & \spaplus (+ GT $\delta$) & 0.56 & 0.54 & 0.29 & 0.15 \\
MiceBone & \spaplus & 0.56 & 0.54 & 0.26 & 0.16 \\
Plankton & GT & 0.91 & 0.35 & 0.20 & 0.07 \\
Plankton & GT+CB & 0.54 & 0.20 & 0.12 & 0.04 \\
Plankton & SPA & 1.71 & 1.39 & 1.00 & 0.59 \\
Plankton & Only BC & 1.71 & 1.65 & 1.28 & 0.77 \\
Plankton & Only CB & 1.00 & 1.75 & 1.74 & 0.77 \\
Plankton & \spaplus (+ GT $\delta$) & 1.10 & 1.12 & 0.85 & 0.50 \\
Plankton & \spaplus & 1.10 & 0.84 & 0.58 & 0.39 \\







     
			
		\end{tabular}
		
\end{table}
}

\newcommand{\tblSimulatedSPASynthetic}{
\begin{table}[tb]
	\caption{
		Simulation of SPA on Synthetic data, full results for visualized median aggregation in \autoref{fig:simulated-0}
	}
 \centering
	\label{tbl:SimulatedSPASynthetic}
		\begin{tabular}{l c c c c c c c c c c c c c c c c}
			\toprule
			

                     
 offset & method & 1 & 3 & 5 & 10 & 20 & 50 & 100 \\
 \midrule
0 & GT & 3.69 & 1.47 & 0.89 & 0.43 & 0.21 & 0.08 & 0.04 \\
0 & GT+CB & 0.91 & 0.35 & 0.21 & 0.12 & 0.07 & 0.05 & 0.04 \\
0 & SPA & 3.67 & 1.46 & 0.90 & 0.43 & 0.20 & 0.08 & 0.03 \\
0 & Only BC & 3.72 & 1.49 & 0.90 & 0.42 & 0.20 & 0.07 & 0.04 \\
0 & Only CB & 0.56 & 0.46 & 0.39 & 0.37 & 0.33 & 0.34 & 0.32 \\
0 & \spaplus (+ GT $\delta$) & 0.90 & 0.34 & 0.21 & 0.12 & 0.07 & 0.05 & 0.04 \\
0 & \spaplus & 0.93 & 0.36 & 0.23 & 0.14 & 0.09 & 0.06 & 0.06 \\
0.1 & GT & 3.67 & 1.46 & 0.89 & 0.44 & 0.21 & 0.08 & 0.04 \\
0.1 & GT+CB & 0.86 & 0.32 & 0.21 & 0.12 & 0.08 & 0.05 & 0.04 \\
0.1 & SPA & 3.95 & 1.58 & 0.94 & 0.46 & 0.22 & 0.10 & 0.06 \\
0.1 & Only BC & 3.92 & 1.56 & 0.96 & 0.51 & 0.25 & 0.10 & 0.05 \\
0.1 & Only CB & 0.58 & 0.47 & 0.41 & 0.37 & 0.35 & 0.33 & 0.32 \\
0.1 & \spaplus (+ GT $\delta$) & 0.94 & 0.36 & 0.24 & 0.14 & 0.09 & 0.06 & 0.04 \\
0.1 & \spaplus & 0.95 & 0.36 & 0.24 & 0.14 & 0.09 & 0.06 & 0.05 \\
0.4 & GT & 3.71 & 1.48 & 0.89 & 0.45 & 0.20 & 0.08 & 0.04 \\
0.4 & GT+CB & 0.87 & 0.34 & 0.22 & 0.12 & 0.08 & 0.05 & 0.04 \\
0.4 & SPA & 4.75 & 2.22 & 1.44 & 0.82 & 0.48 & 0.31 & 0.25 \\
0.4 & Only BC & 4.64 & 2.56 & 1.69 & 0.86 & 0.42 & 0.18 & 0.09 \\
0.4 & Only CB & 0.75 & 0.61 & 0.54 & 0.45 & 0.39 & 0.33 & 0.34 \\
0.4 & \spaplus (+ GT $\delta$) & 1.20 & 0.63 & 0.44 & 0.24 & 0.14 & 0.08 & 0.06 \\
0.4 & \spaplus & 1.21 & 0.62 & 0.46 & 0.31 & 0.26 & 0.21 & 0.19 \\
0.6 & GT & 3.75 & 1.47 & 0.90 & 0.43 & 0.21 & 0.08 & 0.04 \\
0.6 & GT+CB & 0.96 & 0.35 & 0.21 & 0.12 & 0.08 & 0.05 & 0.04 \\
0.6 & SPA & 5.18 & 3.08 & 2.24 & 1.33 & 0.83 & 0.56 & 0.48 \\
0.6 & Only BC & 5.19 & 3.25 & 2.63 & 1.37 & 0.67 & 0.28 & 0.15 \\
0.6 & Only CB & 0.89 & 0.71 & 0.65 & 0.55 & 0.47 & 0.36 & 0.34 \\
0.6 & \spaplus (+ GT $\delta$) & 1.47 & 0.92 & 0.64 & 0.37 & 0.22 & 0.11 & 0.07 \\
0.6 & \spaplus & 1.47 & 0.91 & 0.71 & 0.56 & 0.50 & 0.46 & 0.46 \\


			
		\end{tabular}
		
\end{table}
}

\newcommand{\tblBenchmarkSupervisedMedian}{
\begin{table}[tb]
	\caption{
		Benchmark results  with 100\% in. sup. with median aggregation, metric: KL $\pm$ STD (budget), columns are the number of annotations used, $S$ describes the expected speedup
  }
	\label{tbl:BenchmarkSupervisedMedian}
 \centering
	\resizebox{\linewidth}{!}{
		\begin{tabular}{l c c c c c c c c c c c c c c c c}
			\toprule
	
	method & 1 & 3 & 5 & 10& 20 & 50 & 100 \\
\midrule		
Baseline &0.52 $\pm$ 0.04( 1.00) & 0.34 $\pm$ 0.02( 3.00) & 0.37 $\pm$ 0.03( 5.00) & 0.29 $\pm$ 0.02( 10.00) &   -   &   -   &   -   \\
 DivideMix &0.44 $\pm$ 0.05( 1.00) & 0.47 $\pm$ 0.03( 3.00) & 0.41 $\pm$ 0.04( 5.00) & 0.45 $\pm$ 0.04( 10.00) &   -   &   -   &   -   \\
 Pseudo soft &0.43 $\pm$ 0.07( 1.00) & 0.37 $\pm$ 0.03( 3.00) & 0.34 $\pm$ 0.02( 5.00) & 0.30 $\pm$ 0.02( 10.00) &   -   &   -   &   -   \\
 GT+CB &0.44 $\pm$ 0.03( 1.00) & 0.26 $\pm$ 0.01( 3.00) & 0.25 $\pm$ 0.01( 5.00) & 0.24 $\pm$ 0.01( 10.00) &   -   &   -   &   -   \\
 \spaplus (ours) &0.29 $\pm$ 0.02( 2.00) & 0.28 $\pm$ 0.01( 4.00) & 0.26 $\pm$ 0.02( 6.00) & 0.25 $\pm$ 0.01( 11.00) & 0.27 $\pm$ 0.02( 21.00) & 0.25 $\pm$ 0.02( 51.00) & 0.24 $\pm$ 0.01( 101.00) \\
 \spaplus (ours) $S$=2.5 &0.29 $\pm$ 0.02( 1.40) & 0.28 $\pm$ 0.01( 2.20) & 0.26 $\pm$ 0.02( 3.00) & 0.25 $\pm$ 0.01( 5.00) & 0.27 $\pm$ 0.02( 9.00) & 0.25 $\pm$ 0.02( 21.00) & 0.24 $\pm$ 0.01( 41.00) \\
 \spaplus (ours) $S$=10 &0.29 $\pm$ 0.02( 1.10) & 0.28 $\pm$ 0.01( 1.30) & 0.26 $\pm$ 0.02( 1.50) & 0.25 $\pm$ 0.01( 2.00) & 0.27 $\pm$ 0.02( 3.00) & 0.25 $\pm$ 0.02( 6.00) & 0.24 $\pm$ 0.01( 11.00) \\



		
		\end{tabular}
	}
		
\end{table}
}


\newcommand{\tblBenchmarkSupervisedMean}{
\begin{table}[tb]
	\caption{
		Benchmark results  with 100\% in. sup. with mean aggregation, metric: KL $\pm$ STD (budget), columns are the number of annotations used, $S$ describes the expected speedup
  }
	\label{tbl:BenchmarkSupervisedMean}
 \centering
	\resizebox{\linewidth}{!}{
		\begin{tabular}{l c c c c c c c c c c c c c c c c}
			\toprule
	
	method & 1 & 3 & 5 & 10 & 20 & 50 & 100\\
\midrule		
Baseline &0.69 $\pm$ 0.08( 1.00) & 0.37 $\pm$ 0.04( 3.00) & 0.39 $\pm$ 0.07( 5.00) & 0.33 $\pm$ 0.04( 10.00) &   -   &   -   &   -   \\
 DivideMix &0.52 $\pm$ 0.06( 1.00) & 0.56 $\pm$ 0.11( 3.00) & 0.54 $\pm$ 0.05( 5.00) & 0.64 $\pm$ 0.14( 10.00) &   -   &   -   &   -   \\
 Pseudo soft &0.52 $\pm$ 0.07( 1.00) & 0.39 $\pm$ 0.04( 3.00) & 0.36 $\pm$ 0.03( 5.00) & 0.33 $\pm$ 0.02( 10.00) &   -   &   -   &   -   \\
 GT+CB &0.60 $\pm$ 0.29( 1.00) & 0.32 $\pm$ 0.03( 3.00) & 0.30 $\pm$ 0.01( 5.00) & 0.30 $\pm$ 0.02( 10.00) &   -   &   -   &   -   \\
 \spaplus (ours) &0.37 $\pm$ 0.02( 2.00) & 0.33 $\pm$ 0.02( 4.00) & 0.32 $\pm$ 0.03( 6.00) & 0.30 $\pm$ 0.02( 11.00) & 0.31 $\pm$ 0.03( 21.00) & 0.29 $\pm$ 0.02( 51.00) & 0.29 $\pm$ 0.02( 101.00) \\
 \spaplus (ours) $S$=2.5 &0.37 $\pm$ 0.02( 1.40) & 0.33 $\pm$ 0.02( 2.20) & 0.32 $\pm$ 0.03( 3.00) & 0.30 $\pm$ 0.02( 5.00) & 0.31 $\pm$ 0.03( 9.00) & 0.29 $\pm$ 0.02( 21.00) & 0.29 $\pm$ 0.02( 41.00) \\
 \spaplus (ours) $S$=10 &0.37 $\pm$ 0.02( 1.10) & 0.33 $\pm$ 0.02( 1.30) & 0.32 $\pm$ 0.03( 1.50) & 0.30 $\pm$ 0.02( 2.00) & 0.31 $\pm$ 0.03( 3.00) & 0.29 $\pm$ 0.02( 6.00) & 0.29 $\pm$ 0.02( 11.00) \\


		
		\end{tabular}
	}
		
\end{table}
}

\newcommand{\tblBenchmarkSupervised}{
\begin{table*}[tb]
	\caption{
		Benchmark results  with 100\% in. sup. without aggregation, metric: KL $\pm$ STD (budget), columns are the number of annotations used, $S$ describes the expected speedup
	}
	\label{tbl:BenchmarkSupervised}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{l c c c c c c c c c c c c c c c c}
			\toprule
			
	 dataset & method & 1 & 3 & 5 & 10 & 20 & 50 & 100 \\
	 \midrule
 Benthic & Baseline &1.17 $\pm$ 0.04( 1.00) & 0.81 $\pm$ 0.04( 3.00) & 0.76 $\pm$ 0.04( 5.00) & 0.75 $\pm$ 0.03( 10.00) &   -   &   -   &   -   \\
 Benthic & DivideMix &0.87 $\pm$ 0.07( 1.00) & 0.82 $\pm$ 0.00( 3.00) & 0.84 $\pm$ 0.02( 5.00) & 0.83 $\pm$ 0.05( 10.00) &   -   &   -   &   -   \\
 Benthic & Pseudo soft &1.00 $\pm$ 0.08( 1.00) & 0.76 $\pm$ 0.06( 3.00) & 0.71 $\pm$ 0.05( 5.00) & 0.70 $\pm$ 0.02( 10.00) &   -   &   -   &   -   \\
 Benthic & GT+CB &0.81 $\pm$ 0.04( 1.00) & 0.68 $\pm$ 0.02( 3.00) & 0.67 $\pm$ 0.00( 5.00) & 0.65 $\pm$ 0.01( 10.00) &   -   &   -   &   -   \\
 Benthic & \spaplus (ours) &0.78 $\pm$ 0.03( 2.00) & 0.76 $\pm$ 0.06( 4.00) & 0.71 $\pm$ 0.05( 6.00) & 0.67 $\pm$ 0.02( 11.00) & 0.68 $\pm$ 0.02( 21.00) & 0.67 $\pm$ 0.06( 51.00) & 0.65 $\pm$ 0.03( 101.00) \\
 Benthic & \spaplus (ours) $S$=2.5 &0.78 $\pm$ 0.03( 1.40) & 0.76 $\pm$ 0.06( 2.20) & 0.71 $\pm$ 0.05( 3.00) & 0.67 $\pm$ 0.02( 5.00) & 0.68 $\pm$ 0.02( 9.00) & 0.67 $\pm$ 0.06( 21.00) & 0.65 $\pm$ 0.03( 41.00) \\
 Benthic & \spaplus (ours) $S$=10 &0.78 $\pm$ 0.03( 1.10) & 0.76 $\pm$ 0.06( 1.30) & 0.71 $\pm$ 0.05( 1.50) & 0.67 $\pm$ 0.02( 2.00) & 0.68 $\pm$ 0.02( 3.00) & 0.67 $\pm$ 0.06( 6.00) & 0.65 $\pm$ 0.03( 11.00) \\
 CIFAR10H & Baseline &0.41 $\pm$ 0.02( 1.00) & 0.30 $\pm$ 0.02( 3.00) & 0.27 $\pm$ 0.03( 5.00) & 0.26 $\pm$ 0.02( 10.00) &   -   &   -   &   -   \\
 CIFAR10H & DivideMix &0.36 $\pm$ 0.02( 1.00) & 0.35 $\pm$ 0.01( 3.00) & 0.35 $\pm$ 0.05( 5.00) & 0.37 $\pm$ 0.03( 10.00) &   -   &   -   &   -   \\
 CIFAR10H & Pseudo soft &0.41 $\pm$ 0.02( 1.00) & 0.41 $\pm$ 0.02( 3.00) & 0.42 $\pm$ 0.01( 5.00) & 0.43 $\pm$ 0.02( 10.00) &   -   &   -   &   -   \\
 CIFAR10H & GT+CB &0.27 $\pm$ 0.01( 1.00) & 0.25 $\pm$ 0.01( 3.00) & 0.24 $\pm$ 0.02( 5.00) & 0.25 $\pm$ 0.01( 10.00) &   -   &   -   &   -   \\
 CIFAR10H & \spaplus (ours) &0.25 $\pm$ 0.01( 2.00) & 0.26 $\pm$ 0.01( 4.00) & 0.24 $\pm$ 0.01( 6.00) & 0.24 $\pm$ 0.01( 11.00) & 0.24 $\pm$ 0.01( 21.00) & 0.25 $\pm$ 0.02( 51.00) & 0.24 $\pm$ 0.01( 101.00) \\
 CIFAR10H & \spaplus (ours) $S$=2.5 &0.25 $\pm$ 0.01( 1.40) & 0.26 $\pm$ 0.01( 2.20) & 0.24 $\pm$ 0.01( 3.00) & 0.24 $\pm$ 0.01( 5.00) & 0.24 $\pm$ 0.01( 9.00) & 0.25 $\pm$ 0.02( 21.00) & 0.24 $\pm$ 0.01( 41.00) \\
 CIFAR10H & \spaplus (ours) $S$=10 &0.25 $\pm$ 0.01( 1.10) & 0.26 $\pm$ 0.01( 1.30) & 0.24 $\pm$ 0.01( 1.50) & 0.24 $\pm$ 0.01( 2.00) & 0.24 $\pm$ 0.01( 3.00) & 0.25 $\pm$ 0.02( 6.00) & 0.24 $\pm$ 0.01( 11.00) \\
 MiceBone & Baseline &0.55 $\pm$ 0.06( 1.00) & 0.27 $\pm$ 0.03( 3.00) & 0.27 $\pm$ 0.02( 5.00) & 0.23 $\pm$ 0.02( 10.00) &   -   &   -   &   -   \\
 MiceBone & DivideMix &0.38 $\pm$ 0.05( 1.00) & 0.30 $\pm$ 0.04( 3.00) & 0.34 $\pm$ 0.02( 5.00) & 0.35 $\pm$ 0.05( 10.00) &   -   &   -   &   -   \\
 MiceBone & Pseudo soft &0.40 $\pm$ 0.08( 1.00) & 0.29 $\pm$ 0.03( 3.00) & 0.27 $\pm$ 0.04( 5.00) & 0.22 $\pm$ 0.02( 10.00) &   -   &   -   &   -   \\
 MiceBone & GT+CB &0.35 $\pm$ 0.05( 1.00) & 0.24 $\pm$ 0.01( 3.00) & 0.25 $\pm$ 0.01( 5.00) & 0.23 $\pm$ 0.02( 10.00) &   -   &   -   &   -   \\
 MiceBone & \spaplus (ours) &0.31 $\pm$ 0.03( 2.00) & 0.30 $\pm$ 0.00( 4.00) & 0.27 $\pm$ 0.01( 6.00) & 0.26 $\pm$ 0.04( 11.00) & 0.25 $\pm$ 0.04( 21.00) & 0.25 $\pm$ 0.02( 51.00) & 0.23 $\pm$ 0.03( 101.00) \\
 MiceBone & \spaplus (ours) $S$=2.5 &0.31 $\pm$ 0.03( 1.40) & 0.30 $\pm$ 0.00( 2.20) & 0.27 $\pm$ 0.01( 3.00) & 0.26 $\pm$ 0.04( 5.00) & 0.25 $\pm$ 0.04( 9.00) & 0.25 $\pm$ 0.02( 21.00) & 0.23 $\pm$ 0.03( 41.00) \\
 MiceBone & \spaplus (ours) $S$=10 &0.31 $\pm$ 0.03( 1.10) & 0.30 $\pm$ 0.00( 1.30) & 0.27 $\pm$ 0.01( 1.50) & 0.26 $\pm$ 0.04( 2.00) & 0.25 $\pm$ 0.04( 3.00) & 0.25 $\pm$ 0.02( 6.00) & 0.23 $\pm$ 0.03( 11.00) \\
 Pig & Baseline &0.75 $\pm$ 0.05( 1.00) & 0.56 $\pm$ 0.02( 3.00) & 0.62 $\pm$ 0.04( 5.00) & 0.54 $\pm$ 0.04( 10.00) &   -   &   -   &   -   \\
 Pig & DivideMix &0.95 $\pm$ 0.04( 1.00) & 1.11 $\pm$ 0.32( 3.00) & 1.36 $\pm$ 0.19( 5.00) & 1.04 $\pm$ 0.25( 10.00) &   -   &   -   &   -   \\
 Pig & Pseudo soft &0.70 $\pm$ 0.06( 1.00) & 0.63 $\pm$ 0.03( 3.00) & 0.59 $\pm$ 0.04( 5.00) & 0.61 $\pm$ 0.07( 10.00) &   -   &   -   &   -   \\
 Pig & GT+CB &0.67 $\pm$ 0.08( 1.00) & 0.55 $\pm$ 0.01( 3.00) & 0.51 $\pm$ 0.01( 5.00) & 0.51 $\pm$ 0.04( 10.00) &   -   &   -   &   -   \\
 Pig & \spaplus (ours) &0.61 $\pm$ 0.02( 2.00) & 0.54 $\pm$ 0.02( 4.00) & 0.62 $\pm$ 0.14( 6.00) & 0.51 $\pm$ 0.00( 11.00) & 0.58 $\pm$ 0.08( 21.00) & 0.50 $\pm$ 0.02( 51.00) & 0.50 $\pm$ 0.02( 101.00) \\
 Pig & \spaplus (ours) $S$=2.5 &0.61 $\pm$ 0.02( 1.40) & 0.54 $\pm$ 0.02( 2.20) & 0.62 $\pm$ 0.14( 3.00) & 0.51 $\pm$ 0.00( 5.00) & 0.58 $\pm$ 0.08( 9.00) & 0.50 $\pm$ 0.02( 21.00) & 0.50 $\pm$ 0.02( 41.00) \\
 Pig & \spaplus (ours) $S$=10 &0.61 $\pm$ 0.02( 1.10) & 0.54 $\pm$ 0.02( 1.30) & 0.62 $\pm$ 0.14( 1.50) & 0.51 $\pm$ 0.00( 2.00) & 0.58 $\pm$ 0.08( 3.00) & 0.50 $\pm$ 0.02( 6.00) & 0.50 $\pm$ 0.02( 11.00) \\
 Plankton & Baseline &0.34 $\pm$ 0.02( 1.00) & 0.23 $\pm$ 0.02( 3.00) & 0.22 $\pm$ 0.01( 5.00) & 0.20 $\pm$ 0.02( 10.00) &   -   &   -   &   -   \\
 Plankton & DivideMix &0.34 $\pm$ 0.01( 1.00) & 0.34 $\pm$ 0.01( 3.00) & 0.34 $\pm$ 0.01( 5.00) & 0.34 $\pm$ 0.01( 10.00) &   -   &   -   &   -   \\
 Plankton & Pseudo soft &0.32 $\pm$ 0.06( 1.00) & 0.33 $\pm$ 0.08( 3.00) & 0.24 $\pm$ 0.03( 5.00) & 0.25 $\pm$ 0.01( 10.00) &   -   &   -   &   -   \\
 Plankton & GT+CB &0.25 $\pm$ 0.01( 1.00) & 0.21 $\pm$ 0.02( 3.00) & 0.20 $\pm$ 0.01( 5.00) & 0.20 $\pm$ 0.01( 10.00) &   -   &   -   &   -   \\
 Plankton & \spaplus (ours) &0.26 $\pm$ 0.01( 2.00) & 0.23 $\pm$ 0.01( 4.00) & 0.23 $\pm$ 0.01( 6.00) & 0.22 $\pm$ 0.01( 11.00) & 0.22 $\pm$ 0.01( 21.00) & 0.22 $\pm$ 0.01( 51.00) & 0.22 $\pm$ 0.01( 101.00) \\
 Plankton & \spaplus (ours) $S$=2.5 &0.26 $\pm$ 0.01( 1.40) & 0.23 $\pm$ 0.01( 2.20) & 0.23 $\pm$ 0.01( 3.00) & 0.22 $\pm$ 0.01( 5.00) & 0.22 $\pm$ 0.01( 9.00) & 0.22 $\pm$ 0.01( 21.00) & 0.22 $\pm$ 0.01( 41.00) \\
 Plankton & \spaplus (ours) $S$=10 &0.26 $\pm$ 0.01( 1.10) & 0.23 $\pm$ 0.01( 1.30) & 0.23 $\pm$ 0.01( 1.50) & 0.22 $\pm$ 0.01( 2.00) & 0.22 $\pm$ 0.01( 3.00) & 0.22 $\pm$ 0.01( 6.00) & 0.22 $\pm$ 0.01( 11.00) \\
 QualityMRI & Baseline &1.73 $\pm$ 0.48( 1.00) & 0.39 $\pm$ 0.19( 3.00) & 0.52 $\pm$ 0.28( 5.00) & 0.31 $\pm$ 0.14( 10.00) &   -   &   -   &   -   \\
 QualityMRI & DivideMix &0.46 $\pm$ 0.26( 1.00) & 0.60 $\pm$ 0.58( 3.00) & 0.17 $\pm$ 0.05( 5.00) & 1.34 $\pm$ 0.84( 10.00) &   -   &   -   &   -   \\
 QualityMRI & Pseudo soft &0.62 $\pm$ 0.16( 1.00) & 0.21 $\pm$ 0.10( 3.00) & 0.28 $\pm$ 0.03( 5.00) & 0.12 $\pm$ 0.04( 10.00) &   -   &   -   &   -   \\
 QualityMRI & GT+CB &0.47 $\pm$ 0.10( 1.00) & 0.22 $\pm$ 0.17( 3.00) & 0.15 $\pm$ 0.01( 5.00) & 0.24 $\pm$ 0.13( 10.00) &   -   &   -   &   -   \\
 QualityMRI & \spaplus (ours) &0.24 $\pm$ 0.09( 2.00) & 0.12 $\pm$ 0.03( 4.00) & 0.11 $\pm$ 0.07( 6.00) & 0.11 $\pm$ 0.05( 11.00) & 0.10 $\pm$ 0.04( 21.00) & 0.12 $\pm$ 0.04( 51.00) & 0.16 $\pm$ 0.04( 101.00) \\
 QualityMRI & \spaplus (ours) $S$=2.5 &0.24 $\pm$ 0.09( 1.40) & 0.12 $\pm$ 0.03( 2.20) & 0.11 $\pm$ 0.07( 3.00) & 0.11 $\pm$ 0.05( 5.00) & 0.10 $\pm$ 0.04( 9.00) & 0.12 $\pm$ 0.04( 21.00) & 0.16 $\pm$ 0.04( 41.00) \\
 QualityMRI & \spaplus (ours) $S$=10 &0.24 $\pm$ 0.09( 1.10) & 0.12 $\pm$ 0.03( 1.30) & 0.11 $\pm$ 0.07( 1.50) & 0.11 $\pm$ 0.05( 2.00) & 0.10 $\pm$ 0.04( 3.00) & 0.12 $\pm$ 0.04( 6.00) & 0.16 $\pm$ 0.04( 11.00) \\
 Synthetic & Baseline &0.08 $\pm$ 0.01( 1.00) & 0.05 $\pm$ 0.00( 3.00) & 0.06 $\pm$ 0.01( 5.00) & 0.04 $\pm$ 0.00( 10.00) &   -   &   -   &   -   \\
 Synthetic & DivideMix &0.33 $\pm$ 0.00( 1.00) & 0.48 $\pm$ 0.06( 3.00) & 0.42 $\pm$ 0.07( 5.00) & 0.43 $\pm$ 0.04( 10.00) &   -   &   -   &   -   \\
 Synthetic & Pseudo soft &0.10 $\pm$ 0.01( 1.00) & 0.07 $\pm$ 0.00( 3.00) & 0.08 $\pm$ 0.01( 5.00) & 0.06 $\pm$ 0.01( 10.00) &   -   &   -   &   -   \\
 Synthetic & GT+CB &0.10 $\pm$ 0.00( 1.00) & 0.08 $\pm$ 0.00( 3.00) & 0.07 $\pm$ 0.01( 5.00) & 0.07 $\pm$ 0.00( 10.00) &   -   &   -   &   -   \\
 Synthetic & \spaplus (ours) &0.08 $\pm$ 0.01( 2.00) & 0.07 $\pm$ 0.01( 4.00) & 0.08 $\pm$ 0.00( 6.00) & 0.08 $\pm$ 0.00( 11.00) & 0.08 $\pm$ 0.00( 21.00) & 0.07 $\pm$ 0.01( 51.00) & 0.07 $\pm$ 0.00( 101.00) \\
 Synthetic & \spaplus (ours) $S$=2.5 &0.08 $\pm$ 0.01( 1.40) & 0.07 $\pm$ 0.01( 2.20) & 0.08 $\pm$ 0.00( 3.00) & 0.08 $\pm$ 0.00( 5.00) & 0.08 $\pm$ 0.00( 9.00) & 0.07 $\pm$ 0.01( 21.00) & 0.07 $\pm$ 0.00( 41.00) \\
 Synthetic & \spaplus (ours) $S$=10 &0.08 $\pm$ 0.01( 1.10) & 0.07 $\pm$ 0.01( 1.30) & 0.08 $\pm$ 0.00( 1.50) & 0.08 $\pm$ 0.00( 2.00) & 0.08 $\pm$ 0.00( 3.00) & 0.07 $\pm$ 0.01( 6.00) & 0.07 $\pm$ 0.00( 11.00) \\
 Treeversity\#1 & Baseline &0.49 $\pm$ 0.04( 1.00) & 0.37 $\pm$ 0.01( 3.00) & 0.37 $\pm$ 0.00( 5.00) & 0.36 $\pm$ 0.02( 10.00) &   -   &   -   &   -   \\
 Treeversity\#1 & DivideMix &0.47 $\pm$ 0.01( 1.00) & 0.46 $\pm$ 0.01( 3.00) & 0.46 $\pm$ 0.01( 5.00) & 0.46 $\pm$ 0.01( 10.00) &   -   &   -   &   -   \\
 Treeversity\#1 & Pseudo soft &0.46 $\pm$ 0.01( 1.00) & 0.41 $\pm$ 0.02( 3.00) & 0.39 $\pm$ 0.02( 5.00) & 0.37 $\pm$ 0.02( 10.00) &   -   &   -   &   -   \\
 Treeversity\#1 & GT+CB &0.41 $\pm$ 0.01( 1.00) & 0.37 $\pm$ 0.02( 3.00) & 0.35 $\pm$ 0.02( 5.00) & 0.36 $\pm$ 0.02( 10.00) &   -   &   -   &   -   \\
 Treeversity\#1 & \spaplus (ours) &0.39 $\pm$ 0.02( 2.00) & 0.37 $\pm$ 0.01( 4.00) & 0.37 $\pm$ 0.02( 6.00) & 0.35 $\pm$ 0.01( 11.00) & 0.35 $\pm$ 0.01( 21.00) & 0.35 $\pm$ 0.02( 51.00) & 0.35 $\pm$ 0.01( 101.00) \\
 Treeversity\#1 & \spaplus (ours) $S$=2.5 &0.39 $\pm$ 0.02( 1.40) & 0.37 $\pm$ 0.01( 2.20) & 0.37 $\pm$ 0.02( 3.00) & 0.35 $\pm$ 0.01( 5.00) & 0.35 $\pm$ 0.01( 9.00) & 0.35 $\pm$ 0.02( 21.00) & 0.35 $\pm$ 0.01( 41.00) \\
 Treeversity\#1 & \spaplus (ours) $S$=10 &0.39 $\pm$ 0.02( 1.10) & 0.37 $\pm$ 0.01( 1.30) & 0.37 $\pm$ 0.02( 1.50) & 0.35 $\pm$ 0.01( 2.00) & 0.35 $\pm$ 0.01( 3.00) & 0.35 $\pm$ 0.02( 6.00) & 0.35 $\pm$ 0.01( 11.00) \\
 Treeversity\#6 & Baseline &1.02 $\pm$ 0.03( 1.00) & 0.50 $\pm$ 0.02( 3.00) & 0.38 $\pm$ 0.00( 5.00) & 0.33 $\pm$ 0.01( 10.00) &   -   &   -   &   -   \\
 Treeversity\#6 & DivideMix &0.62 $\pm$ 0.05( 1.00) & 0.71 $\pm$ 0.02( 3.00) & 0.70 $\pm$ 0.04( 5.00) & 0.77 $\pm$ 0.03( 10.00) &   -   &   -   &   -   \\
 Treeversity\#6 & Pseudo soft &0.83 $\pm$ 0.13( 1.00) & 0.47 $\pm$ 0.02( 3.00) & 0.40 $\pm$ 0.02( 5.00) & 0.35 $\pm$ 0.01( 10.00) &   -   &   -   &   -   \\
 Treeversity\#6 & GT+CB &0.61 $\pm$ 0.03( 1.00) & 0.37 $\pm$ 0.00( 3.00) & 0.33 $\pm$ 0.01( 5.00) & 0.31 $\pm$ 0.00( 10.00) &   -   &   -   &   -   \\
 Treeversity\#6 & \spaplus (ours) &0.47 $\pm$ 0.01( 2.00) & 0.37 $\pm$ 0.02( 4.00) & 0.34 $\pm$ 0.02( 6.00) & 0.33 $\pm$ 0.01( 11.00) & 0.30 $\pm$ 0.01( 21.00) & 0.30 $\pm$ 0.01( 51.00) & 0.28 $\pm$ 0.00( 101.00) \\
 Treeversity\#6 & \spaplus (ours) $S$=2.5 &0.47 $\pm$ 0.01( 1.40) & 0.37 $\pm$ 0.02( 2.20) & 0.34 $\pm$ 0.02( 3.00) & 0.33 $\pm$ 0.01( 5.00) & 0.30 $\pm$ 0.01( 9.00) & 0.30 $\pm$ 0.01( 21.00) & 0.28 $\pm$ 0.00( 41.00) \\
 Treeversity\#6 & \spaplus (ours) $S$=10 &0.47 $\pm$ 0.01( 1.10) & 0.37 $\pm$ 0.02( 1.30) & 0.34 $\pm$ 0.02( 1.50) & 0.33 $\pm$ 0.01( 2.00) & 0.30 $\pm$ 0.01( 3.00) & 0.30 $\pm$ 0.01( 6.00) & 0.28 $\pm$ 0.00( 11.00) \\
 Turkey & Baseline &0.40 $\pm$ 0.08( 1.00) & 0.27 $\pm$ 0.01( 3.00) & 0.38 $\pm$ 0.24( 5.00) & 0.24 $\pm$ 0.06( 10.00) &   -   &   -   &   -   \\
 Turkey & DivideMix &0.43 $\pm$ 0.08( 1.00) & 0.46 $\pm$ 0.04( 3.00) & 0.39 $\pm$ 0.06( 5.00) & 0.41 $\pm$ 0.07( 10.00) &   -   &   -   &   -   \\
 Turkey & Pseudo soft &0.37 $\pm$ 0.08( 1.00) & 0.28 $\pm$ 0.05( 3.00) & 0.22 $\pm$ 0.02( 5.00) & 0.21 $\pm$ 0.02( 10.00) &   -   &   -   &   -   \\
 Turkey & GT+CB &2.09 $\pm$ 2.55( 1.00) & 0.26 $\pm$ 0.04( 3.00) & 0.22 $\pm$ 0.01( 5.00) & 0.19 $\pm$ 0.01( 10.00) &   -   &   -   &   -   \\
 Turkey & \spaplus (ours) &0.27 $\pm$ 0.00( 2.00) & 0.25 $\pm$ 0.01( 4.00) & 0.23 $\pm$ 0.02( 6.00) & 0.22 $\pm$ 0.02( 11.00) & 0.28 $\pm$ 0.10( 21.00) & 0.20 $\pm$ 0.02( 51.00) & 0.19 $\pm$ 0.01( 101.00) \\
 Turkey & \spaplus (ours) $S$=2.5 &0.27 $\pm$ 0.00( 1.40) & 0.25 $\pm$ 0.01( 2.20) & 0.23 $\pm$ 0.02( 3.00) & 0.22 $\pm$ 0.02( 5.00) & 0.28 $\pm$ 0.10( 9.00) & 0.20 $\pm$ 0.02( 21.00) & 0.19 $\pm$ 0.01( 41.00) \\
 Turkey & \spaplus (ours) $S$=10 &0.27 $\pm$ 0.00( 1.10) & 0.25 $\pm$ 0.01( 1.30) & 0.23 $\pm$ 0.02( 1.50) & 0.22 $\pm$ 0.02( 2.00) & 0.28 $\pm$ 0.10( 3.00) & 0.20 $\pm$ 0.02( 6.00) & 0.19 $\pm$ 0.01( 11.00) \\

		
			
		\end{tabular}
	}
		
\end{table*}
}

\newcommand{\tblBenchmarkSemiSupervised}{
\begin{table*}[tb]
	\caption{
		Benchmark results  with 20, 50 and 100\% in. sup. without aggregation, metric: KL $\pm$ STD (budget), columns are the number of annotations used, $S$ describes the expected speedup, best viewed in digital form
	}
	\label{tbl:BenchmarkSemiSupervised}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{l c | c c c c | c c c c c  | c c c c c c}
			\toprule

   in. sup. & & 20\% & & & & 50 \% & & & & & 100\% \\
			
		dataset & method & 1 & 3 & 5 & 10 & 1 & 2 & 3 & 5 & 10 & 1 & 3 & 5 & 10 \\
  \midrule 
Benthic & Baseline &1.55 $\pm$ 0.08( 0.20) &   -   & 1.09 $\pm$ 0.03( 1.00) &   -   & 1.34 $\pm$ 0.08( 0.50) & 1.08 $\pm$ 0.10( 1.00) &   -   &   -   &   -   & 1.17 $\pm$ 0.04( 1.00) & 0.81 $\pm$ 0.04( 3.00) & 0.76 $\pm$ 0.04( 5.00) & 0.75 $\pm$ 0.03( 10.00) \\
 Benthic & DivideMix &0.99 $\pm$ 0.07( 0.20) &   -   & 1.06 $\pm$ 0.08( 1.00) &   -   & 0.83 $\pm$ 0.03( 0.50) & 1.06 $\pm$ 0.03( 1.00) &   -   &   -   &   -   & 0.87 $\pm$ 0.07( 1.00) & 0.82 $\pm$ 0.00( 3.00) & 0.84 $\pm$ 0.02( 5.00) & 0.83 $\pm$ 0.05( 10.00) \\
 Benthic & Pseudo soft &1.08 $\pm$ 0.05( 0.20) &   -   & 0.81 $\pm$ 0.02( 1.00) &   -   & 1.01 $\pm$ 0.02( 0.50) & 0.83 $\pm$ 0.05( 1.00) &   -   &   -   &   -   & 1.00 $\pm$ 0.08( 1.00) & 0.76 $\pm$ 0.06( 3.00) & 0.71 $\pm$ 0.05( 5.00) & 0.70 $\pm$ 0.02( 10.00) \\
 Benthic & GT+CB &  -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   & 0.81 $\pm$ 0.04( 1.00) & 0.68 $\pm$ 0.02( 3.00) & 0.67 $\pm$ 0.00( 5.00) & 0.65 $\pm$ 0.01( 10.00) \\
 Benthic & \spaplus (inc. un.) &1.00 $\pm$ 0.12( 1.20) & 0.77 $\pm$ 0.04( 3.20) & 0.74 $\pm$ 0.05( 5.20) & 0.69 $\pm$ 0.05( 10.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Benthic & \spaplus (ours) &0.92 $\pm$ 0.06( 0.40) & 0.95 $\pm$ 0.06( 0.80) & 0.88 $\pm$ 0.05( 1.20) & 0.91 $\pm$ 0.05( 2.20) & 0.79 $\pm$ 0.02( 1.00) &   -   & 0.90 $\pm$ 0.21( 2.00) & 0.72 $\pm$ 0.03( 3.00) & 0.74 $\pm$ 0.03( 5.50) & 0.78 $\pm$ 0.03( 2.00) & 0.76 $\pm$ 0.06( 4.00) & 0.71 $\pm$ 0.05( 6.00) & 0.67 $\pm$ 0.02( 11.00) \\
 Benthic & \spaplus (inc. un.) $S$=2.5 &1.00 $\pm$ 0.12( 0.60) & 0.77 $\pm$ 0.04( 1.40) & 0.74 $\pm$ 0.05( 2.20) & 0.69 $\pm$ 0.05( 4.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Benthic & \spaplus (inc. un.) $S$=10 &1.00 $\pm$ 0.12( 0.30) & 0.77 $\pm$ 0.04( 0.50) & 0.74 $\pm$ 0.05( 0.70) & 0.69 $\pm$ 0.05( 1.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Benthic & \spaplus (ours) $S$=2.5 &0.92 $\pm$ 0.06( 0.28) & 0.95 $\pm$ 0.06( 0.44) & 0.88 $\pm$ 0.05( 0.60) & 0.91 $\pm$ 0.05( 1.00) & 0.79 $\pm$ 0.02( 0.70) &   -   & 0.90 $\pm$ 0.21( 1.10) & 0.72 $\pm$ 0.03( 1.50) & 0.74 $\pm$ 0.03( 2.50) & 0.78 $\pm$ 0.03( 1.40) & 0.76 $\pm$ 0.06( 2.20) & 0.71 $\pm$ 0.05( 3.00) & 0.67 $\pm$ 0.02( 5.00) \\
 Benthic & \spaplus (ours) $S$=10 &0.92 $\pm$ 0.06( 0.22) & 0.95 $\pm$ 0.06( 0.26) & 0.88 $\pm$ 0.05( 0.30) & 0.91 $\pm$ 0.05( 0.40) & 0.79 $\pm$ 0.02( 0.55) &   -   & 0.90 $\pm$ 0.21( 0.65) & 0.72 $\pm$ 0.03( 0.75) & 0.74 $\pm$ 0.03( 1.00) & 0.78 $\pm$ 0.03( 1.10) & 0.76 $\pm$ 0.06( 1.30) & 0.71 $\pm$ 0.05( 1.50) & 0.67 $\pm$ 0.02( 2.00) \\
 CIFAR10H & Baseline &0.63 $\pm$ 0.01( 0.20) &   -   & 0.55 $\pm$ 0.01( 1.00) &   -   & 0.47 $\pm$ 0.02( 0.50) & 0.38 $\pm$ 0.01( 1.00) &   -   &   -   &   -   & 0.41 $\pm$ 0.02( 1.00) & 0.30 $\pm$ 0.02( 3.00) & 0.27 $\pm$ 0.03( 5.00) & 0.26 $\pm$ 0.02( 10.00) \\
 CIFAR10H & DivideMix &0.67 $\pm$ 0.02( 0.20) &   -   & 0.65 $\pm$ 0.13( 1.00) &   -   & 0.44 $\pm$ 0.03( 0.50) & 0.36 $\pm$ 0.01( 1.00) &   -   &   -   &   -   & 0.36 $\pm$ 0.02( 1.00) & 0.35 $\pm$ 0.01( 3.00) & 0.35 $\pm$ 0.05( 5.00) & 0.37 $\pm$ 0.03( 10.00) \\
 CIFAR10H & Pseudo soft &1.12 $\pm$ 0.03( 0.20) &   -   & 1.10 $\pm$ 0.03( 1.00) &   -   & 0.69 $\pm$ 0.02( 0.50) & 0.71 $\pm$ 0.07( 1.00) &   -   &   -   &   -   & 0.41 $\pm$ 0.02( 1.00) & 0.41 $\pm$ 0.02( 3.00) & 0.42 $\pm$ 0.01( 5.00) & 0.43 $\pm$ 0.02( 10.00) \\
 CIFAR10H & GT+CB &  -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   & 0.27 $\pm$ 0.01( 1.00) & 0.25 $\pm$ 0.01( 3.00) & 0.24 $\pm$ 0.02( 5.00) & 0.25 $\pm$ 0.01( 10.00) \\
 CIFAR10H & \spaplus (inc. un.) &0.29 $\pm$ 0.01( 1.20) & 0.26 $\pm$ 0.01( 3.20) & 0.25 $\pm$ 0.01( 5.20) & 0.24 $\pm$ 0.02( 10.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 CIFAR10H & \spaplus (ours) &0.55 $\pm$ 0.01( 0.40) & 0.56 $\pm$ 0.01( 0.80) & 0.56 $\pm$ 0.04( 1.20) & 0.56 $\pm$ 0.02( 2.20) & 0.34 $\pm$ 0.02( 1.00) &   -   & 0.35 $\pm$ 0.03( 2.00) & 0.32 $\pm$ 0.01( 3.00) & 0.35 $\pm$ 0.01( 5.50) & 0.25 $\pm$ 0.01( 2.00) & 0.26 $\pm$ 0.01( 4.00) & 0.24 $\pm$ 0.01( 6.00) & 0.24 $\pm$ 0.01( 11.00) \\
 CIFAR10H & \spaplus (inc. un.) $S$=2.5 &0.29 $\pm$ 0.01( 0.60) & 0.26 $\pm$ 0.01( 1.40) & 0.25 $\pm$ 0.01( 2.20) & 0.24 $\pm$ 0.02( 4.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 CIFAR10H & \spaplus (inc. un.) $S$=10 &0.29 $\pm$ 0.01( 0.30) & 0.26 $\pm$ 0.01( 0.50) & 0.25 $\pm$ 0.01( 0.70) & 0.24 $\pm$ 0.02( 1.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 CIFAR10H & \spaplus (ours) $S$=2.5 &0.55 $\pm$ 0.01( 0.28) & 0.56 $\pm$ 0.01( 0.44) & 0.56 $\pm$ 0.04( 0.60) & 0.56 $\pm$ 0.02( 1.00) & 0.34 $\pm$ 0.02( 0.70) &   -   & 0.35 $\pm$ 0.03( 1.10) & 0.32 $\pm$ 0.01( 1.50) & 0.35 $\pm$ 0.01( 2.50) & 0.25 $\pm$ 0.01( 1.40) & 0.26 $\pm$ 0.01( 2.20) & 0.24 $\pm$ 0.01( 3.00) & 0.24 $\pm$ 0.01( 5.00) \\
 CIFAR10H & \spaplus (ours) $S$=10 &0.55 $\pm$ 0.01( 0.22) & 0.56 $\pm$ 0.01( 0.26) & 0.56 $\pm$ 0.04( 0.30) & 0.56 $\pm$ 0.02( 0.40) & 0.34 $\pm$ 0.02( 0.55) &   -   & 0.35 $\pm$ 0.03( 0.65) & 0.32 $\pm$ 0.01( 0.75) & 0.35 $\pm$ 0.01( 1.00) & 0.25 $\pm$ 0.01( 1.10) & 0.26 $\pm$ 0.01( 1.30) & 0.24 $\pm$ 0.01( 1.50) & 0.24 $\pm$ 0.01( 2.00) \\
 MiceBone & Baseline &0.56 $\pm$ 0.06( 0.20) &   -   & 0.34 $\pm$ 0.03( 1.00) &   -   & 0.53 $\pm$ 0.07( 0.50) & 0.39 $\pm$ 0.01( 1.00) &   -   &   -   &   -   & 0.55 $\pm$ 0.06( 1.00) & 0.27 $\pm$ 0.03( 3.00) & 0.27 $\pm$ 0.02( 5.00) & 0.23 $\pm$ 0.02( 10.00) \\
 MiceBone & DivideMix &0.42 $\pm$ 0.06( 0.20) &   -   & 0.47 $\pm$ 0.10( 1.00) &   -   & 0.38 $\pm$ 0.04( 0.50) & 0.51 $\pm$ 0.12( 1.00) &   -   &   -   &   -   & 0.38 $\pm$ 0.05( 1.00) & 0.30 $\pm$ 0.04( 3.00) & 0.34 $\pm$ 0.02( 5.00) & 0.35 $\pm$ 0.05( 10.00) \\
 MiceBone & Pseudo soft &0.46 $\pm$ 0.05( 0.20) &   -   & 0.28 $\pm$ 0.03( 1.00) &   -   & 0.48 $\pm$ 0.07( 0.50) & 0.34 $\pm$ 0.07( 1.00) &   -   &   -   &   -   & 0.40 $\pm$ 0.08( 1.00) & 0.29 $\pm$ 0.03( 3.00) & 0.27 $\pm$ 0.04( 5.00) & 0.22 $\pm$ 0.02( 10.00) \\
 MiceBone & GT+CB &  -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   & 0.35 $\pm$ 0.05( 1.00) & 0.24 $\pm$ 0.01( 3.00) & 0.25 $\pm$ 0.01( 5.00) & 0.23 $\pm$ 0.02( 10.00) \\
 MiceBone & \spaplus (inc. un.) &0.37 $\pm$ 0.05( 1.20) & 0.31 $\pm$ 0.03( 3.20) & 0.30 $\pm$ 0.02( 5.20) & 0.27 $\pm$ 0.02( 10.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 MiceBone & \spaplus (ours) &0.33 $\pm$ 0.03( 0.40) & 0.33 $\pm$ 0.03( 0.80) & 0.33 $\pm$ 0.05( 1.20) & 0.34 $\pm$ 0.05( 2.20) & 0.32 $\pm$ 0.06( 1.00) &   -   & 0.31 $\pm$ 0.03( 2.00) & 0.28 $\pm$ 0.03( 3.00) & 0.30 $\pm$ 0.04( 5.50) & 0.31 $\pm$ 0.03( 2.00) & 0.30 $\pm$ 0.00( 4.00) & 0.27 $\pm$ 0.01( 6.00) & 0.26 $\pm$ 0.04( 11.00) \\
 MiceBone & \spaplus (inc. un.) $S$=2.5 &0.37 $\pm$ 0.05( 0.60) & 0.31 $\pm$ 0.03( 1.40) & 0.30 $\pm$ 0.02( 2.20) & 0.27 $\pm$ 0.02( 4.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 MiceBone & \spaplus (inc. un.) $S$=10 &0.37 $\pm$ 0.05( 0.30) & 0.31 $\pm$ 0.03( 0.50) & 0.30 $\pm$ 0.02( 0.70) & 0.27 $\pm$ 0.02( 1.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 MiceBone & \spaplus (ours) $S$=2.5 &0.33 $\pm$ 0.03( 0.28) & 0.33 $\pm$ 0.03( 0.44) & 0.33 $\pm$ 0.05( 0.60) & 0.34 $\pm$ 0.05( 1.00) & 0.32 $\pm$ 0.06( 0.70) &   -   & 0.31 $\pm$ 0.03( 1.10) & 0.28 $\pm$ 0.03( 1.50) & 0.30 $\pm$ 0.04( 2.50) & 0.31 $\pm$ 0.03( 1.40) & 0.30 $\pm$ 0.00( 2.20) & 0.27 $\pm$ 0.01( 3.00) & 0.26 $\pm$ 0.04( 5.00) \\
 MiceBone & \spaplus (ours) $S$=10 &0.33 $\pm$ 0.03( 0.22) & 0.33 $\pm$ 0.03( 0.26) & 0.33 $\pm$ 0.05( 0.30) & 0.34 $\pm$ 0.05( 0.40) & 0.32 $\pm$ 0.06( 0.55) &   -   & 0.31 $\pm$ 0.03( 0.65) & 0.28 $\pm$ 0.03( 0.75) & 0.30 $\pm$ 0.04( 1.00) & 0.31 $\pm$ 0.03( 1.10) & 0.30 $\pm$ 0.00( 1.30) & 0.27 $\pm$ 0.01( 1.50) & 0.26 $\pm$ 0.04( 2.00) \\
 Pig & Baseline &0.79 $\pm$ 0.06( 0.20) &   -   & 0.61 $\pm$ 0.01( 1.00) &   -   & 0.79 $\pm$ 0.05( 0.50) & 0.62 $\pm$ 0.07( 1.00) &   -   &   -   &   -   & 0.75 $\pm$ 0.05( 1.00) & 0.56 $\pm$ 0.02( 3.00) & 0.62 $\pm$ 0.04( 5.00) & 0.54 $\pm$ 0.04( 10.00) \\
 Pig & DivideMix &0.84 $\pm$ 0.05( 0.20) &   -   & 0.86 $\pm$ 0.17( 1.00) &   -   & 0.94 $\pm$ 0.07( 0.50) & 1.11 $\pm$ 0.18( 1.00) &   -   &   -   &   -   & 0.95 $\pm$ 0.04( 1.00) & 1.11 $\pm$ 0.32( 3.00) & 1.36 $\pm$ 0.19( 5.00) & 1.04 $\pm$ 0.25( 10.00) \\
 Pig & Pseudo soft &0.74 $\pm$ 0.10( 0.20) &   -   & 0.61 $\pm$ 0.03( 1.00) &   -   & 0.68 $\pm$ 0.08( 0.50) & 0.67 $\pm$ 0.01( 1.00) &   -   &   -   &   -   & 0.70 $\pm$ 0.06( 1.00) & 0.63 $\pm$ 0.03( 3.00) & 0.59 $\pm$ 0.04( 5.00) & 0.61 $\pm$ 0.07( 10.00) \\
 Pig & GT+CB &  -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   & 0.67 $\pm$ 0.08( 1.00) & 0.55 $\pm$ 0.01( 3.00) & 0.51 $\pm$ 0.01( 5.00) & 0.51 $\pm$ 0.04( 10.00) \\
 Pig & \spaplus (inc. un.) &0.72 $\pm$ 0.02( 1.20) & 0.55 $\pm$ 0.02( 3.20) & 0.55 $\pm$ 0.01( 5.20) & 0.54 $\pm$ 0.02( 10.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Pig & \spaplus (ours) &0.68 $\pm$ 0.03( 0.40) & 0.62 $\pm$ 0.06( 0.80) & 0.66 $\pm$ 0.04( 1.20) & 0.69 $\pm$ 0.11( 2.20) & 0.60 $\pm$ 0.06( 1.00) &   -   & 0.62 $\pm$ 0.06( 2.00) & 0.58 $\pm$ 0.01( 3.00) & 0.57 $\pm$ 0.03( 5.50) & 0.61 $\pm$ 0.02( 2.00) & 0.54 $\pm$ 0.02( 4.00) & 0.62 $\pm$ 0.14( 6.00) & 0.51 $\pm$ 0.00( 11.00) \\
 Pig & \spaplus (inc. un.) $S$=2.5 &0.72 $\pm$ 0.02( 0.60) & 0.55 $\pm$ 0.02( 1.40) & 0.55 $\pm$ 0.01( 2.20) & 0.54 $\pm$ 0.02( 4.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Pig & \spaplus (inc. un.) $S$=10 &0.72 $\pm$ 0.02( 0.30) & 0.55 $\pm$ 0.02( 0.50) & 0.55 $\pm$ 0.01( 0.70) & 0.54 $\pm$ 0.02( 1.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Pig & \spaplus (ours) $S$=2.5 &0.68 $\pm$ 0.03( 0.28) & 0.62 $\pm$ 0.06( 0.44) & 0.66 $\pm$ 0.04( 0.60) & 0.69 $\pm$ 0.11( 1.00) & 0.60 $\pm$ 0.06( 0.70) &   -   & 0.62 $\pm$ 0.06( 1.10) & 0.58 $\pm$ 0.01( 1.50) & 0.57 $\pm$ 0.03( 2.50) & 0.61 $\pm$ 0.02( 1.40) & 0.54 $\pm$ 0.02( 2.20) & 0.62 $\pm$ 0.14( 3.00) & 0.51 $\pm$ 0.00( 5.00) \\
 Pig & \spaplus (ours) $S$=10 &0.68 $\pm$ 0.03( 0.22) & 0.62 $\pm$ 0.06( 0.26) & 0.66 $\pm$ 0.04( 0.30) & 0.69 $\pm$ 0.11( 0.40) & 0.60 $\pm$ 0.06( 0.55) &   -   & 0.62 $\pm$ 0.06( 0.65) & 0.58 $\pm$ 0.01( 0.75) & 0.57 $\pm$ 0.03( 1.00) & 0.61 $\pm$ 0.02( 1.10) & 0.54 $\pm$ 0.02( 1.30) & 0.62 $\pm$ 0.14( 1.50) & 0.51 $\pm$ 0.00( 2.00) \\
 Plankton & Baseline &0.43 $\pm$ 0.01( 0.20) &   -   & 0.34 $\pm$ 0.03( 1.00) &   -   & 0.36 $\pm$ 0.03( 0.50) & 0.28 $\pm$ 0.02( 1.00) &   -   &   -   &   -   & 0.34 $\pm$ 0.02( 1.00) & 0.23 $\pm$ 0.02( 3.00) & 0.22 $\pm$ 0.01( 5.00) & 0.20 $\pm$ 0.02( 10.00) \\
 Plankton & DivideMix &0.48 $\pm$ 0.03( 0.20) &   -   & 0.48 $\pm$ 0.02( 1.00) &   -   & 0.35 $\pm$ 0.02( 0.50) & 0.44 $\pm$ 0.03( 1.00) &   -   &   -   &   -   & 0.34 $\pm$ 0.01( 1.00) & 0.34 $\pm$ 0.01( 3.00) & 0.34 $\pm$ 0.01( 5.00) & 0.34 $\pm$ 0.01( 10.00) \\
 Plankton & Pseudo soft &0.41 $\pm$ 0.05( 0.20) &   -   & 0.32 $\pm$ 0.04( 1.00) &   -   & 0.44 $\pm$ 0.13( 0.50) & 0.46 $\pm$ 0.20( 1.00) &   -   &   -   &   -   & 0.32 $\pm$ 0.06( 1.00) & 0.33 $\pm$ 0.08( 3.00) & 0.24 $\pm$ 0.03( 5.00) & 0.25 $\pm$ 0.01( 10.00) \\
 Plankton & GT+CB &  -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   & 0.25 $\pm$ 0.01( 1.00) & 0.21 $\pm$ 0.02( 3.00) & 0.20 $\pm$ 0.01( 5.00) & 0.20 $\pm$ 0.01( 10.00) \\
 Plankton & \spaplus (inc. un.) &0.37 $\pm$ 0.01( 1.20) & 0.30 $\pm$ 0.01( 3.20) & 0.30 $\pm$ 0.02( 5.20) & 0.28 $\pm$ 0.02( 10.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Plankton & \spaplus (ours) &0.41 $\pm$ 0.02( 0.40) & 0.41 $\pm$ 0.02( 0.80) & 0.41 $\pm$ 0.02( 1.20) & 0.42 $\pm$ 0.03( 2.20) & 0.28 $\pm$ 0.02( 1.00) &   -   & 0.27 $\pm$ 0.02( 2.00) & 0.27 $\pm$ 0.02( 3.00) & 0.27 $\pm$ 0.02( 5.50) & 0.26 $\pm$ 0.01( 2.00) & 0.23 $\pm$ 0.01( 4.00) & 0.23 $\pm$ 0.01( 6.00) & 0.22 $\pm$ 0.01( 11.00) \\
 Plankton & \spaplus (inc. un.) $S$=2.5 &0.37 $\pm$ 0.01( 0.60) & 0.30 $\pm$ 0.01( 1.40) & 0.30 $\pm$ 0.02( 2.20) & 0.28 $\pm$ 0.02( 4.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Plankton & \spaplus (inc. un.) $S$=10 &0.37 $\pm$ 0.01( 0.30) & 0.30 $\pm$ 0.01( 0.50) & 0.30 $\pm$ 0.02( 0.70) & 0.28 $\pm$ 0.02( 1.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Plankton & \spaplus (ours) $S$=2.5 &0.41 $\pm$ 0.02( 0.28) & 0.41 $\pm$ 0.02( 0.44) & 0.41 $\pm$ 0.02( 0.60) & 0.42 $\pm$ 0.03( 1.00) & 0.28 $\pm$ 0.02( 0.70) &   -   & 0.27 $\pm$ 0.02( 1.10) & 0.27 $\pm$ 0.02( 1.50) & 0.27 $\pm$ 0.02( 2.50) & 0.26 $\pm$ 0.01( 1.40) & 0.23 $\pm$ 0.01( 2.20) & 0.23 $\pm$ 0.01( 3.00) & 0.22 $\pm$ 0.01( 5.00) \\
 Plankton & \spaplus (ours) $S$=10 &0.41 $\pm$ 0.02( 0.22) & 0.41 $\pm$ 0.02( 0.26) & 0.41 $\pm$ 0.02( 0.30) & 0.42 $\pm$ 0.03( 0.40) & 0.28 $\pm$ 0.02( 0.55) &   -   & 0.27 $\pm$ 0.02( 0.65) & 0.27 $\pm$ 0.02( 0.75) & 0.27 $\pm$ 0.02( 1.00) & 0.26 $\pm$ 0.01( 1.10) & 0.23 $\pm$ 0.01( 1.30) & 0.23 $\pm$ 0.01( 1.50) & 0.22 $\pm$ 0.01( 2.00) \\
 QualityMRI & Baseline &3.12 $\pm$ 1.42( 0.20) &   -   & 0.56 $\pm$ 0.25( 1.00) &   -   & 1.12 $\pm$ 0.36( 0.50) & 0.41 $\pm$ 0.31( 1.00) &   -   &   -   &   -   & 1.73 $\pm$ 0.48( 1.00) & 0.39 $\pm$ 0.19( 3.00) & 0.52 $\pm$ 0.28( 5.00) & 0.31 $\pm$ 0.14( 10.00) \\
 QualityMRI & DivideMix &0.24 $\pm$ 0.13( 0.20) &   -   & 0.26 $\pm$ 0.07( 1.00) &   -   & 0.45 $\pm$ 0.38( 0.50) & 0.91 $\pm$ 0.32( 1.00) &   -   &   -   &   -   & 0.46 $\pm$ 0.26( 1.00) & 0.60 $\pm$ 0.58( 3.00) & 0.17 $\pm$ 0.05( 5.00) & 1.34 $\pm$ 0.84( 10.00) \\
 QualityMRI & Pseudo soft &2.78 $\pm$ 0.67( 0.20) &   -   & 0.20 $\pm$ 0.04( 1.00) &   -   & 1.16 $\pm$ 0.34( 0.50) & 0.65 $\pm$ 0.38( 1.00) &   -   &   -   &   -   & 0.62 $\pm$ 0.16( 1.00) & 0.21 $\pm$ 0.10( 3.00) & 0.28 $\pm$ 0.03( 5.00) & 0.12 $\pm$ 0.04( 10.00) \\
 QualityMRI & GT+CB &  -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   & 0.47 $\pm$ 0.10( 1.00) & 0.22 $\pm$ 0.17( 3.00) & 0.15 $\pm$ 0.01( 5.00) & 0.24 $\pm$ 0.13( 10.00) \\
 QualityMRI & \spaplus (inc. un.) &0.22 $\pm$ 0.14( 1.20) & 0.14 $\pm$ 0.08( 3.20) & 0.08 $\pm$ 0.00( 5.20) & 0.10 $\pm$ 0.03( 10.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 QualityMRI & \spaplus (ours) &0.24 $\pm$ 0.10( 0.40) & 0.16 $\pm$ 0.04( 0.80) & 0.14 $\pm$ 0.02( 1.20) & 0.17 $\pm$ 0.05( 2.20) & 0.38 $\pm$ 0.12( 1.00) &   -   & 0.24 $\pm$ 0.10( 2.00) & 0.16 $\pm$ 0.07( 3.00) & 0.38 $\pm$ 0.10( 5.50) & 0.24 $\pm$ 0.09( 2.00) & 0.12 $\pm$ 0.03( 4.00) & 0.11 $\pm$ 0.07( 6.00) & 0.11 $\pm$ 0.05( 11.00) \\
 QualityMRI & \spaplus (inc. un.) $S$=2.5 &0.22 $\pm$ 0.14( 0.60) & 0.14 $\pm$ 0.08( 1.40) & 0.08 $\pm$ 0.00( 2.20) & 0.10 $\pm$ 0.03( 4.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 QualityMRI & \spaplus (inc. un.) $S$=10 &0.22 $\pm$ 0.14( 0.30) & 0.14 $\pm$ 0.08( 0.50) & 0.08 $\pm$ 0.00( 0.70) & 0.10 $\pm$ 0.03( 1.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 QualityMRI & \spaplus (ours) $S$=2.5 &0.24 $\pm$ 0.10( 0.28) & 0.16 $\pm$ 0.04( 0.44) & 0.14 $\pm$ 0.02( 0.60) & 0.17 $\pm$ 0.05( 1.00) & 0.38 $\pm$ 0.12( 0.70) &   -   & 0.24 $\pm$ 0.10( 1.10) & 0.16 $\pm$ 0.07( 1.50) & 0.38 $\pm$ 0.10( 2.50) & 0.24 $\pm$ 0.09( 1.40) & 0.12 $\pm$ 0.03( 2.20) & 0.11 $\pm$ 0.07( 3.00) & 0.11 $\pm$ 0.05( 5.00) \\
 QualityMRI & \spaplus (ours) $S$=10 &0.24 $\pm$ 0.10( 0.22) & 0.16 $\pm$ 0.04( 0.26) & 0.14 $\pm$ 0.02( 0.30) & 0.17 $\pm$ 0.05( 0.40) & 0.38 $\pm$ 0.12( 0.55) &   -   & 0.24 $\pm$ 0.10( 0.65) & 0.16 $\pm$ 0.07( 0.75) & 0.38 $\pm$ 0.10( 1.00) & 0.24 $\pm$ 0.09( 1.10) & 0.12 $\pm$ 0.03( 1.30) & 0.11 $\pm$ 0.07( 1.50) & 0.11 $\pm$ 0.05( 2.00) \\
 Synthetic & Baseline &0.16 $\pm$ 0.02( 0.20) &   -   & 0.07 $\pm$ 0.01( 1.00) &   -   & 0.12 $\pm$ 0.02( 0.50) & 0.08 $\pm$ 0.01( 1.00) &   -   &   -   &   -   & 0.08 $\pm$ 0.01( 1.00) & 0.05 $\pm$ 0.00( 3.00) & 0.06 $\pm$ 0.01( 5.00) & 0.04 $\pm$ 0.00( 10.00) \\
 Synthetic & DivideMix &0.25 $\pm$ 0.02( 0.20) &   -   & 0.71 $\pm$ 0.10( 1.00) &   -   & 0.28 $\pm$ 0.02( 0.50) & 1.03 $\pm$ 0.07( 1.00) &   -   &   -   &   -   & 0.33 $\pm$ 0.00( 1.00) & 0.48 $\pm$ 0.06( 3.00) & 0.42 $\pm$ 0.07( 5.00) & 0.43 $\pm$ 0.04( 10.00) \\
 Synthetic & Pseudo soft &0.32 $\pm$ 0.06( 0.20) &   -   & 0.11 $\pm$ 0.03( 1.00) &   -   & 0.13 $\pm$ 0.02( 0.50) & 0.11 $\pm$ 0.02( 1.00) &   -   &   -   &   -   & 0.10 $\pm$ 0.01( 1.00) & 0.07 $\pm$ 0.00( 3.00) & 0.08 $\pm$ 0.01( 5.00) & 0.06 $\pm$ 0.01( 10.00) \\
 Synthetic & GT+CB &  -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   & 0.10 $\pm$ 0.00( 1.00) & 0.08 $\pm$ 0.00( 3.00) & 0.07 $\pm$ 0.01( 5.00) & 0.07 $\pm$ 0.00( 10.00) \\
 Synthetic & \spaplus (inc. un.) &0.11 $\pm$ 0.02( 1.20) & 0.10 $\pm$ 0.01( 3.20) & 0.09 $\pm$ 0.00( 5.20) & 0.08 $\pm$ 0.01( 10.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Synthetic & \spaplus (ours) &0.18 $\pm$ 0.01( 0.40) & 0.18 $\pm$ 0.01( 0.80) & 0.17 $\pm$ 0.01( 1.20) & 0.17 $\pm$ 0.01( 2.20) & 0.12 $\pm$ 0.01( 1.00) &   -   & 0.12 $\pm$ 0.01( 2.00) & 0.12 $\pm$ 0.01( 3.00) & 0.12 $\pm$ 0.00( 5.50) & 0.08 $\pm$ 0.01( 2.00) & 0.07 $\pm$ 0.01( 4.00) & 0.08 $\pm$ 0.00( 6.00) & 0.08 $\pm$ 0.00( 11.00) \\
 Synthetic & \spaplus (inc. un.) $S$=2.5 &0.11 $\pm$ 0.02( 0.60) & 0.10 $\pm$ 0.01( 1.40) & 0.09 $\pm$ 0.00( 2.20) & 0.08 $\pm$ 0.01( 4.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Synthetic & \spaplus (inc. un.) $S$=10 &0.11 $\pm$ 0.02( 0.30) & 0.10 $\pm$ 0.01( 0.50) & 0.09 $\pm$ 0.00( 0.70) & 0.08 $\pm$ 0.01( 1.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Synthetic & \spaplus (ours) $S$=2.5 &0.18 $\pm$ 0.01( 0.28) & 0.18 $\pm$ 0.01( 0.44) & 0.17 $\pm$ 0.01( 0.60) & 0.17 $\pm$ 0.01( 1.00) & 0.12 $\pm$ 0.01( 0.70) &   -   & 0.12 $\pm$ 0.01( 1.10) & 0.12 $\pm$ 0.01( 1.50) & 0.12 $\pm$ 0.00( 2.50) & 0.08 $\pm$ 0.01( 1.40) & 0.07 $\pm$ 0.01( 2.20) & 0.08 $\pm$ 0.00( 3.00) & 0.08 $\pm$ 0.00( 5.00) \\
 Synthetic & \spaplus (ours) $S$=10 &0.18 $\pm$ 0.01( 0.22) & 0.18 $\pm$ 0.01( 0.26) & 0.17 $\pm$ 0.01( 0.30) & 0.17 $\pm$ 0.01( 0.40) & 0.12 $\pm$ 0.01( 0.55) &   -   & 0.12 $\pm$ 0.01( 0.65) & 0.12 $\pm$ 0.01( 0.75) & 0.12 $\pm$ 0.00( 1.00) & 0.08 $\pm$ 0.01( 1.10) & 0.07 $\pm$ 0.01( 1.30) & 0.08 $\pm$ 0.00( 1.50) & 0.08 $\pm$ 0.00( 2.00) \\
 Treeversity\#1 & Baseline &0.55 $\pm$ 0.01( 0.20) &   -   & 0.51 $\pm$ 0.01( 1.00) &   -   & 0.46 $\pm$ 0.03( 0.50) & 0.43 $\pm$ 0.03( 1.00) &   -   &   -   &   -   & 0.49 $\pm$ 0.04( 1.00) & 0.37 $\pm$ 0.01( 3.00) & 0.37 $\pm$ 0.00( 5.00) & 0.36 $\pm$ 0.02( 10.00) \\
 Treeversity\#1 & DivideMix &0.53 $\pm$ 0.00( 0.20) &   -   & 0.63 $\pm$ 0.02( 1.00) &   -   & 0.47 $\pm$ 0.01( 0.50) & 0.60 $\pm$ 0.03( 1.00) &   -   &   -   &   -   & 0.47 $\pm$ 0.01( 1.00) & 0.46 $\pm$ 0.01( 3.00) & 0.46 $\pm$ 0.01( 5.00) & 0.46 $\pm$ 0.01( 10.00) \\
 Treeversity\#1 & Pseudo soft &0.70 $\pm$ 0.06( 0.20) &   -   & 0.54 $\pm$ 0.01( 1.00) &   -   & 0.53 $\pm$ 0.03( 0.50) & 0.50 $\pm$ 0.02( 1.00) &   -   &   -   &   -   & 0.46 $\pm$ 0.01( 1.00) & 0.41 $\pm$ 0.02( 3.00) & 0.39 $\pm$ 0.02( 5.00) & 0.37 $\pm$ 0.02( 10.00) \\
 Treeversity\#1 & GT+CB &  -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   & 0.41 $\pm$ 0.01( 1.00) & 0.37 $\pm$ 0.02( 3.00) & 0.35 $\pm$ 0.02( 5.00) & 0.36 $\pm$ 0.02( 10.00) \\
 Treeversity\#1 & \spaplus (inc. un.) &0.44 $\pm$ 0.02( 1.20) & 0.38 $\pm$ 0.02( 3.20) & 0.37 $\pm$ 0.02( 5.20) & 0.38 $\pm$ 0.02( 10.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Treeversity\#1 & \spaplus (ours) &0.49 $\pm$ 0.02( 0.40) & 0.50 $\pm$ 0.01( 0.80) & 0.50 $\pm$ 0.02( 1.20) & 0.50 $\pm$ 0.02( 2.20) & 0.42 $\pm$ 0.01( 1.00) &   -   & 0.41 $\pm$ 0.02( 2.00) & 0.41 $\pm$ 0.01( 3.00) & 0.40 $\pm$ 0.00( 5.50) & 0.39 $\pm$ 0.02( 2.00) & 0.37 $\pm$ 0.01( 4.00) & 0.37 $\pm$ 0.02( 6.00) & 0.35 $\pm$ 0.01( 11.00) \\
 Treeversity\#1 & \spaplus (inc. un.) $S$=2.5 &0.44 $\pm$ 0.02( 0.60) & 0.38 $\pm$ 0.02( 1.40) & 0.37 $\pm$ 0.02( 2.20) & 0.38 $\pm$ 0.02( 4.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Treeversity\#1 & \spaplus (inc. un.) $S$=10 &0.44 $\pm$ 0.02( 0.30) & 0.38 $\pm$ 0.02( 0.50) & 0.37 $\pm$ 0.02( 0.70) & 0.38 $\pm$ 0.02( 1.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Treeversity\#1 & \spaplus (ours) $S$=2.5 &0.49 $\pm$ 0.02( 0.28) & 0.50 $\pm$ 0.01( 0.44) & 0.50 $\pm$ 0.02( 0.60) & 0.50 $\pm$ 0.02( 1.00) & 0.42 $\pm$ 0.01( 0.70) &   -   & 0.41 $\pm$ 0.02( 1.10) & 0.41 $\pm$ 0.01( 1.50) & 0.40 $\pm$ 0.00( 2.50) & 0.39 $\pm$ 0.02( 1.40) & 0.37 $\pm$ 0.01( 2.20) & 0.37 $\pm$ 0.02( 3.00) & 0.35 $\pm$ 0.01( 5.00) \\
 Treeversity\#1 & \spaplus (ours) $S$=10 &0.49 $\pm$ 0.02( 0.22) & 0.50 $\pm$ 0.01( 0.26) & 0.50 $\pm$ 0.02( 0.30) & 0.50 $\pm$ 0.02( 0.40) & 0.42 $\pm$ 0.01( 0.55) &   -   & 0.41 $\pm$ 0.02( 0.65) & 0.41 $\pm$ 0.01( 0.75) & 0.40 $\pm$ 0.00( 1.00) & 0.39 $\pm$ 0.02( 1.10) & 0.37 $\pm$ 0.01( 1.30) & 0.37 $\pm$ 0.02( 1.50) & 0.35 $\pm$ 0.01( 2.00) \\
 Treeversity\#6 & Baseline &1.42 $\pm$ 0.14( 0.20) &   -   & 0.46 $\pm$ 0.01( 1.00) &   -   & 1.29 $\pm$ 0.09( 0.50) & 0.64 $\pm$ 0.01( 1.00) &   -   &   -   &   -   & 1.02 $\pm$ 0.03( 1.00) & 0.50 $\pm$ 0.02( 3.00) & 0.38 $\pm$ 0.00( 5.00) & 0.33 $\pm$ 0.01( 10.00) \\
 Treeversity\#6 & DivideMix &0.55 $\pm$ 0.05( 0.20) &   -   & 0.88 $\pm$ 0.04( 1.00) &   -   & 0.54 $\pm$ 0.05( 0.50) & 1.03 $\pm$ 0.09( 1.00) &   -   &   -   &   -   & 0.62 $\pm$ 0.05( 1.00) & 0.71 $\pm$ 0.02( 3.00) & 0.70 $\pm$ 0.04( 5.00) & 0.77 $\pm$ 0.03( 10.00) \\
 Treeversity\#6 & Pseudo soft &0.97 $\pm$ 0.10( 0.20) &   -   & 0.49 $\pm$ 0.04( 1.00) &   -   & 0.85 $\pm$ 0.04( 0.50) & 0.60 $\pm$ 0.02( 1.00) &   -   &   -   &   -   & 0.83 $\pm$ 0.13( 1.00) & 0.47 $\pm$ 0.02( 3.00) & 0.40 $\pm$ 0.02( 5.00) & 0.35 $\pm$ 0.01( 10.00) \\
 Treeversity\#6 & GT+CB &  -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   & 0.61 $\pm$ 0.03( 1.00) & 0.37 $\pm$ 0.00( 3.00) & 0.33 $\pm$ 0.01( 5.00) & 0.31 $\pm$ 0.00( 10.00) \\
 Treeversity\#6 & \spaplus (inc. un.) &0.69 $\pm$ 0.04( 1.20) & 0.42 $\pm$ 0.01( 3.20) & 0.36 $\pm$ 0.01( 5.20) & 0.32 $\pm$ 0.00( 10.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Treeversity\#6 & \spaplus (ours) &0.47 $\pm$ 0.00( 0.40) & 0.45 $\pm$ 0.00( 0.80) & 0.45 $\pm$ 0.01( 1.20) & 0.45 $\pm$ 0.02( 2.20) & 0.44 $\pm$ 0.01( 1.00) &   -   & 0.41 $\pm$ 0.02( 2.00) & 0.38 $\pm$ 0.02( 3.00) & 0.37 $\pm$ 0.01( 5.50) & 0.47 $\pm$ 0.01( 2.00) & 0.37 $\pm$ 0.02( 4.00) & 0.34 $\pm$ 0.02( 6.00) & 0.33 $\pm$ 0.01( 11.00) \\
 Treeversity\#6 & \spaplus (inc. un.) $S$=2.5 &0.69 $\pm$ 0.04( 0.60) & 0.42 $\pm$ 0.01( 1.40) & 0.36 $\pm$ 0.01( 2.20) & 0.32 $\pm$ 0.00( 4.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Treeversity\#6 & \spaplus (inc. un.) $S$=10 &0.69 $\pm$ 0.04( 0.30) & 0.42 $\pm$ 0.01( 0.50) & 0.36 $\pm$ 0.01( 0.70) & 0.32 $\pm$ 0.00( 1.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Treeversity\#6 & \spaplus (ours) $S$=2.5 &0.47 $\pm$ 0.00( 0.28) & 0.45 $\pm$ 0.00( 0.44) & 0.45 $\pm$ 0.01( 0.60) & 0.45 $\pm$ 0.02( 1.00) & 0.44 $\pm$ 0.01( 0.70) &   -   & 0.41 $\pm$ 0.02( 1.10) & 0.38 $\pm$ 0.02( 1.50) & 0.37 $\pm$ 0.01( 2.50) & 0.47 $\pm$ 0.01( 1.40) & 0.37 $\pm$ 0.02( 2.20) & 0.34 $\pm$ 0.02( 3.00) & 0.33 $\pm$ 0.01( 5.00) \\
 Treeversity\#6 & \spaplus (ours) $S$=10 &0.47 $\pm$ 0.00( 0.22) & 0.45 $\pm$ 0.00( 0.26) & 0.45 $\pm$ 0.01( 0.30) & 0.45 $\pm$ 0.02( 0.40) & 0.44 $\pm$ 0.01( 0.55) &   -   & 0.41 $\pm$ 0.02( 0.65) & 0.38 $\pm$ 0.02( 0.75) & 0.37 $\pm$ 0.01( 1.00) & 0.47 $\pm$ 0.01( 1.10) & 0.37 $\pm$ 0.02( 1.30) & 0.34 $\pm$ 0.02( 1.50) & 0.33 $\pm$ 0.01( 2.00) \\
 Turkey & Baseline &0.64 $\pm$ 0.16( 0.20) &   -   & 0.32 $\pm$ 0.09( 1.00) &   -   & 0.51 $\pm$ 0.08( 0.50) & 0.43 $\pm$ 0.08( 1.00) &   -   &   -   &   -   & 0.40 $\pm$ 0.08( 1.00) & 0.27 $\pm$ 0.01( 3.00) & 0.38 $\pm$ 0.24( 5.00) & 0.24 $\pm$ 0.06( 10.00) \\
 Turkey & DivideMix &0.52 $\pm$ 0.06( 0.20) &   -   & 0.61 $\pm$ 0.11( 1.00) &   -   & 0.46 $\pm$ 0.07( 0.50) & 0.57 $\pm$ 0.13( 1.00) &   -   &   -   &   -   & 0.43 $\pm$ 0.08( 1.00) & 0.46 $\pm$ 0.04( 3.00) & 0.39 $\pm$ 0.06( 5.00) & 0.41 $\pm$ 0.07( 10.00) \\
 Turkey & Pseudo soft &0.45 $\pm$ 0.07( 0.20) &   -   & 0.27 $\pm$ 0.01( 1.00) &   -   & 0.43 $\pm$ 0.09( 0.50) & 0.30 $\pm$ 0.04( 1.00) &   -   &   -   &   -   & 0.37 $\pm$ 0.08( 1.00) & 0.28 $\pm$ 0.05( 3.00) & 0.22 $\pm$ 0.02( 5.00) & 0.21 $\pm$ 0.02( 10.00) \\
 Turkey & GT+CB &  -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   & 2.09 $\pm$ 2.55( 1.00) & 0.26 $\pm$ 0.04( 3.00) & 0.22 $\pm$ 0.01( 5.00) & 0.19 $\pm$ 0.01( 10.00) \\
 Turkey & \spaplus (inc. un.) &0.42 $\pm$ 0.08( 1.20) & 0.30 $\pm$ 0.11( 3.20) & 0.23 $\pm$ 0.01( 5.20) & 0.22 $\pm$ 0.02( 10.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Turkey & \spaplus (ours) &0.44 $\pm$ 0.07( 0.40) & 0.42 $\pm$ 0.08( 0.80) & 0.41 $\pm$ 0.07( 1.20) & 0.43 $\pm$ 0.03( 2.20) & 0.36 $\pm$ 0.09( 1.00) &   -   & 0.30 $\pm$ 0.06( 2.00) & 0.29 $\pm$ 0.04( 3.00) & 0.35 $\pm$ 0.07( 5.50) & 0.27 $\pm$ 0.00( 2.00) & 0.25 $\pm$ 0.01( 4.00) & 0.23 $\pm$ 0.02( 6.00) & 0.22 $\pm$ 0.02( 11.00) \\
 Turkey & \spaplus (inc. un.) $S$=2.5 &0.42 $\pm$ 0.08( 0.60) & 0.30 $\pm$ 0.11( 1.40) & 0.23 $\pm$ 0.01( 2.20) & 0.22 $\pm$ 0.02( 4.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Turkey & \spaplus (inc. un.) $S$=10 &0.42 $\pm$ 0.08( 0.30) & 0.30 $\pm$ 0.11( 0.50) & 0.23 $\pm$ 0.01( 0.70) & 0.22 $\pm$ 0.02( 1.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 Turkey & \spaplus (ours) $S$=2.5 &0.44 $\pm$ 0.07( 0.28) & 0.42 $\pm$ 0.08( 0.44) & 0.41 $\pm$ 0.07( 0.60) & 0.43 $\pm$ 0.03( 1.00) & 0.36 $\pm$ 0.09( 0.70) &   -   & 0.30 $\pm$ 0.06( 1.10) & 0.29 $\pm$ 0.04( 1.50) & 0.35 $\pm$ 0.07( 2.50) & 0.27 $\pm$ 0.00( 1.40) & 0.25 $\pm$ 0.01( 2.20) & 0.23 $\pm$ 0.02( 3.00) & 0.22 $\pm$ 0.02( 5.00) \\
 Turkey & \spaplus (ours) $S$=10 &0.44 $\pm$ 0.07( 0.22) & 0.42 $\pm$ 0.08( 0.26) & 0.41 $\pm$ 0.07( 0.30) & 0.43 $\pm$ 0.03( 0.40) & 0.36 $\pm$ 0.09( 0.55) &   -   & 0.30 $\pm$ 0.06( 0.65) & 0.29 $\pm$ 0.04( 0.75) & 0.35 $\pm$ 0.07( 1.00) & 0.27 $\pm$ 0.00( 1.10) & 0.25 $\pm$ 0.01( 1.30) & 0.23 $\pm$ 0.02( 1.50) & 0.22 $\pm$ 0.02( 2.00) \\

			
		\end{tabular}
	}
		
\end{table*}
}

\newcommand{\tblBenchmarkSemiSupervisedMedian}{
\begin{table*}[tb]
	\caption{
		Benchmark results  with 20, 50 and 100\% in. sup. with median aggregation, metric: KL $\pm$ STD (budget), columns are the number of annotations used, $S$ describes the expected speedup, best viewed in digital form
	}
	\label{tbl:BenchmarkSemiSupervisedMedian}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{l | c c c c | c c c c c  | c c c c c c}
			\toprule

  in. sup. & 20\% & & & & 50 \% & & & & & 100\% \\
			
		 method & 1 & 3 & 5 & 10 & 1 & 2 & 3 & 5 & 10 & 1 & 3 & 5 & 10 \\
  \midrule 
 Baseline &0.63 $\pm$ 0.06( 0.20) &   -   & 0.49 $\pm$ 0.02( 1.00) &   -   & 0.52 $\pm$ 0.06( 0.50) & 0.42 $\pm$ 0.03( 1.00) &   -   &   -   &   -   & 0.52 $\pm$ 0.04( 1.00) & 0.34 $\pm$ 0.02( 3.00) & 0.37 $\pm$ 0.03( 5.00) & 0.29 $\pm$ 0.02( 10.00) \\
 DivideMix &0.53 $\pm$ 0.05( 0.20) &   -   & 0.64 $\pm$ 0.09( 1.00) &   -   & 0.45 $\pm$ 0.04( 0.50) & 0.75 $\pm$ 0.08( 1.00) &   -   &   -   &   -   & 0.44 $\pm$ 0.05( 1.00) & 0.47 $\pm$ 0.03( 3.00) & 0.41 $\pm$ 0.04( 5.00) & 0.45 $\pm$ 0.04( 10.00) \\
 Pseudo soft &0.72 $\pm$ 0.06( 0.20) &   -   & 0.40 $\pm$ 0.03( 1.00) &   -   & 0.61 $\pm$ 0.06( 0.50) & 0.55 $\pm$ 0.05( 1.00) &   -   &   -   &   -   & 0.43 $\pm$ 0.07( 1.00) & 0.37 $\pm$ 0.03( 3.00) & 0.34 $\pm$ 0.02( 5.00) & 0.30 $\pm$ 0.02( 10.00) \\
 GT+CB &  -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   & 0.44 $\pm$ 0.03( 1.00) & 0.26 $\pm$ 0.01( 3.00) & 0.25 $\pm$ 0.01( 5.00) & 0.24 $\pm$ 0.01( 10.00) \\
 \spaplus (inc. un.) &0.40 $\pm$ 0.03( 1.20) & 0.31 $\pm$ 0.02( 3.20) & 0.30 $\pm$ 0.01( 5.20) & 0.28 $\pm$ 0.02( 10.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 \spaplus (ours) &0.46 $\pm$ 0.02( 0.40) & 0.44 $\pm$ 0.03( 0.80) & 0.43 $\pm$ 0.03( 1.20) & 0.44 $\pm$ 0.03( 2.20) & 0.37 $\pm$ 0.02( 1.00) &   -   & 0.33 $\pm$ 0.03( 2.00) & 0.31 $\pm$ 0.02( 3.00) & 0.36 $\pm$ 0.02( 5.50) & 0.29 $\pm$ 0.02( 2.00) & 0.28 $\pm$ 0.01( 4.00) & 0.26 $\pm$ 0.02( 6.00) & 0.25 $\pm$ 0.01( 11.00) \\
 \spaplus (inc. un.) $S$=2.5 &0.40 $\pm$ 0.03( 0.60) & 0.31 $\pm$ 0.02( 1.40) & 0.30 $\pm$ 0.01( 2.20) & 0.28 $\pm$ 0.02( 4.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 \spaplus (inc. un.) $S$=10 &0.40 $\pm$ 0.03( 0.30) & 0.31 $\pm$ 0.02( 0.50) & 0.30 $\pm$ 0.01( 0.70) & 0.28 $\pm$ 0.02( 1.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 \spaplus (ours) $S$=2.5 &0.46 $\pm$ 0.02( 0.28) & 0.44 $\pm$ 0.03( 0.44) & 0.43 $\pm$ 0.03( 0.60) & 0.44 $\pm$ 0.03( 1.00) & 0.37 $\pm$ 0.02( 0.70) &   -   & 0.33 $\pm$ 0.03( 1.10) & 0.31 $\pm$ 0.02( 1.50) & 0.36 $\pm$ 0.02( 2.50) & 0.29 $\pm$ 0.02( 1.40) & 0.28 $\pm$ 0.01( 2.20) & 0.26 $\pm$ 0.02( 3.00) & 0.25 $\pm$ 0.01( 5.00) \\
 \spaplus (ours) $S$=10 &0.46 $\pm$ 0.02( 0.22) & 0.44 $\pm$ 0.03( 0.26) & 0.43 $\pm$ 0.03( 0.30) & 0.44 $\pm$ 0.03( 0.40) & 0.37 $\pm$ 0.02( 0.55) &   -   & 0.33 $\pm$ 0.03( 0.65) & 0.31 $\pm$ 0.02( 0.75) & 0.36 $\pm$ 0.02( 1.00) & 0.29 $\pm$ 0.02( 1.10) & 0.28 $\pm$ 0.01( 1.30) & 0.26 $\pm$ 0.02( 1.50) & 0.25 $\pm$ 0.01( 2.00) \\



			
		\end{tabular}
	}
		
\end{table*}
}

\newcommand{\tblBenchmarkSemiSupervisedMean}{
\begin{table*}[tb]
	\caption{
		Benchmark results  with 20, 50 and 100\% in. sup. with mean aggregation, metric: KL $\pm$ STD (budget), columns are the number of annotations used, $S$ describes the expected speedup
	}
	\label{tbl:BenchmarkSemiSupervisedMean}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{l | c c c c | c c c c c  | c c c c c c}
			\toprule

  in. sup. & 20\% & & & & 50 \% & & & & & 100\% \\
			
method & 1 & 3 & 5 & 10 & 1 & 2 & 3 & 5 & 10 & 1 & 3 & 5 & 10 \\
 Baseline &0.98 $\pm$ 0.20( 0.20) &   -   & 0.49 $\pm$ 0.05( 1.00) &   -   & 0.70 $\pm$ 0.08( 0.50) & 0.47 $\pm$ 0.07( 1.00) &   -   &   -   &   -   & 0.69 $\pm$ 0.08( 1.00) & 0.37 $\pm$ 0.04( 3.00) & 0.39 $\pm$ 0.07( 5.00) & 0.33 $\pm$ 0.04( 10.00) \\
 DivideMix &0.55 $\pm$ 0.05( 0.20) &   -   & 0.66 $\pm$ 0.08( 1.00) &   -   & 0.51 $\pm$ 0.07( 0.50) & 0.76 $\pm$ 0.10( 1.00) &   -   &   -   &   -   & 0.52 $\pm$ 0.06( 1.00) & 0.56 $\pm$ 0.11( 3.00) & 0.54 $\pm$ 0.05( 5.00) & 0.64 $\pm$ 0.14( 10.00) \\
 Pseudo soft &0.90 $\pm$ 0.12( 0.20) &   -   & 0.47 $\pm$ 0.03( 1.00) &   -   & 0.64 $\pm$ 0.08( 0.50) & 0.52 $\pm$ 0.09( 1.00) &   -   &   -   &   -   & 0.52 $\pm$ 0.07( 1.00) & 0.39 $\pm$ 0.04( 3.00) & 0.36 $\pm$ 0.03( 5.00) & 0.33 $\pm$ 0.02( 10.00) \\
 GT+CB &  -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   & 0.60 $\pm$ 0.29( 1.00) & 0.32 $\pm$ 0.03( 3.00) & 0.30 $\pm$ 0.01( 5.00) & 0.30 $\pm$ 0.02( 10.00) \\
 \spaplus (inc. un.) &0.46 $\pm$ 0.05( 1.20) & 0.35 $\pm$ 0.03( 3.20) & 0.33 $\pm$ 0.02( 5.20) & 0.31 $\pm$ 0.02( 10.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 \spaplus (ours) &0.47 $\pm$ 0.03( 0.40) & 0.46 $\pm$ 0.03( 0.80) & 0.45 $\pm$ 0.03( 1.20) & 0.46 $\pm$ 0.04( 2.20) & 0.40 $\pm$ 0.04( 1.00) &   -   & 0.39 $\pm$ 0.06( 2.00) & 0.35 $\pm$ 0.02( 3.00) & 0.38 $\pm$ 0.03( 5.50) & 0.37 $\pm$ 0.02( 2.00) & 0.33 $\pm$ 0.02( 4.00) & 0.32 $\pm$ 0.03( 6.00) & 0.30 $\pm$ 0.02( 11.00) \\
 \spaplus (inc. un.) $S$=2.5 &0.46 $\pm$ 0.05( 0.60) & 0.35 $\pm$ 0.03( 1.40) & 0.33 $\pm$ 0.02( 2.20) & 0.31 $\pm$ 0.02( 4.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 \spaplus (inc. un.) $S$=10 &0.46 $\pm$ 0.05( 0.30) & 0.35 $\pm$ 0.03( 0.50) & 0.33 $\pm$ 0.02( 0.70) & 0.31 $\pm$ 0.02( 1.20) &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   &   -   \\
 \spaplus (ours) $S$=2.5 &0.47 $\pm$ 0.03( 0.28) & 0.46 $\pm$ 0.03( 0.44) & 0.45 $\pm$ 0.03( 0.60) & 0.46 $\pm$ 0.04( 1.00) & 0.40 $\pm$ 0.04( 0.70) &   -   & 0.39 $\pm$ 0.06( 1.10) & 0.35 $\pm$ 0.02( 1.50) & 0.38 $\pm$ 0.03( 2.50) & 0.37 $\pm$ 0.02( 1.40) & 0.33 $\pm$ 0.02( 2.20) & 0.32 $\pm$ 0.03( 3.00) & 0.30 $\pm$ 0.02( 5.00) \\
 \spaplus (ours) $S$=10 &0.47 $\pm$ 0.03( 0.22) & 0.46 $\pm$ 0.03( 0.26) & 0.45 $\pm$ 0.03( 0.30) & 0.46 $\pm$ 0.04( 0.40) & 0.40 $\pm$ 0.04( 0.55) &   -   & 0.39 $\pm$ 0.06( 0.65) & 0.35 $\pm$ 0.02( 0.75) & 0.38 $\pm$ 0.03( 1.00) & 0.37 $\pm$ 0.02( 1.10) & 0.33 $\pm$ 0.02( 1.30) & 0.32 $\pm$ 0.03( 1.50) & 0.30 $\pm$ 0.02( 2.00) \\

			
		\end{tabular}
	}
		
\end{table*}
}







\newcommand{\tblBenchmarkAblationFirstPart}{
\begin{table*}[tb]
	\caption{
		Benchmark results ablation study,  metric: $KL$ $\pm$ STD, columns are the number of annotations used
	}
	\label{tbl:BenchmarkAblationFirstPart}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{l c c c c c c c c c c c c c c c c}
			\toprule
			
		dataset & method &  1 & 3 & 5 & 10 & 20 & 50 & 100 \\

  \midrule 
  
 Benthic & \spaplus (ours) &0.78 $\pm$ 0.03 & 0.76 $\pm$ 0.06 & 0.71 $\pm$ 0.05 & 0.67 $\pm$ 0.02 & 0.68 $\pm$ 0.02 & 0.67 $\pm$ 0.06 & 0.65 $\pm$ 0.03 \\
 Benthic & \spaplus (+ GT $\delta$) &0.80 $\pm$ 0.03 & 0.78 $\pm$ 0.02 & 0.72 $\pm$ 0.07 & 0.67 $\pm$ 0.04 & 0.69 $\pm$ 0.03 & 0.67 $\pm$ 0.03 & 0.65 $\pm$ 0.02 \\
 Benthic & Only CB &0.79 $\pm$ 0.05 & 0.75 $\pm$ 0.03 & 0.68 $\pm$ 0.01 & 0.70 $\pm$ 0.02 & 0.65 $\pm$ 0.03 & 0.67 $\pm$ 0.03 & 0.69 $\pm$ 0.02 \\
 Benthic & Only CB ($\mu$=0.25) &0.82 $\pm$ 0.05 & 0.76 $\pm$ 0.01 & 0.74 $\pm$ 0.03 & 0.72 $\pm$ 0.03 &   -   &   -   &   -   \\
 Benthic & Only BC &  -   & 0.97 $\pm$ 0.20 & 0.76 $\pm$ 0.05 & 0.71 $\pm$ 0.02 &   -   &   -   &   -   \\
 CIFAR10H & \spaplus (ours) &0.25 $\pm$ 0.01 & 0.26 $\pm$ 0.01 & 0.24 $\pm$ 0.01 & 0.24 $\pm$ 0.01 & 0.24 $\pm$ 0.01 & 0.25 $\pm$ 0.02 & 0.24 $\pm$ 0.01 \\
 CIFAR10H & \spaplus (+ GT $\delta$) &0.26 $\pm$ 0.01 & 0.25 $\pm$ 0.00 & 0.25 $\pm$ 0.01 & 0.25 $\pm$ 0.02 & 0.24 $\pm$ 0.01 & 0.23 $\pm$ 0.01 & 0.24 $\pm$ 0.01 \\
 CIFAR10H & Only CB &0.25 $\pm$ 0.02 & 0.25 $\pm$ 0.01 & 0.24 $\pm$ 0.01 & 0.25 $\pm$ 0.01 & 0.24 $\pm$ 0.01 & 0.25 $\pm$ 0.01 & 0.25 $\pm$ 0.01 \\
 CIFAR10H & Only CB ($\mu$=0.25) &0.30 $\pm$ 0.02 & 0.28 $\pm$ 0.01 & 0.28 $\pm$ 0.01 & 0.28 $\pm$ 0.01 &   -   &   -   &   -   \\
 CIFAR10H & Only BC &  -   & 0.28 $\pm$ 0.01 & 0.27 $\pm$ 0.02 & 0.26 $\pm$ 0.02 &   -   &   -   &   -   \\
 MiceBone & \spaplus (ours) &0.31 $\pm$ 0.03 & 0.30 $\pm$ 0.00 & 0.27 $\pm$ 0.01 & 0.26 $\pm$ 0.04 & 0.25 $\pm$ 0.04 & 0.25 $\pm$ 0.02 & 0.23 $\pm$ 0.03 \\
 MiceBone & \spaplus (+ GT $\delta$) &0.31 $\pm$ 0.02 & 0.29 $\pm$ 0.01 & 0.27 $\pm$ 0.05 & 0.25 $\pm$ 0.01 & 0.24 $\pm$ 0.02 & 0.23 $\pm$ 0.02 & 0.23 $\pm$ 0.02 \\
 MiceBone & Only CB &0.36 $\pm$ 0.04 & 0.28 $\pm$ 0.04 & 0.27 $\pm$ 0.02 & 0.25 $\pm$ 0.05 & 0.25 $\pm$ 0.02 & 0.24 $\pm$ 0.02 & 0.25 $\pm$ 0.04 \\
 MiceBone & Only CB ($\mu$=0.25) &0.34 $\pm$ 0.04 & 0.29 $\pm$ 0.01 & 0.30 $\pm$ 0.03 & 0.30 $\pm$ 0.01 &   -   &   -   &   -   \\
 MiceBone & Only BC &  -   & 0.32 $\pm$ 0.04 & 0.32 $\pm$ 0.02 & 0.26 $\pm$ 0.02 &   -   &   -   &   -   \\
 Pig & \spaplus (ours) &0.61 $\pm$ 0.02 & 0.54 $\pm$ 0.02 & 0.62 $\pm$ 0.14 & 0.51 $\pm$ 0.00 & 0.58 $\pm$ 0.08 & 0.50 $\pm$ 0.02 & 0.50 $\pm$ 0.02 \\
 Pig & \spaplus (+ GT $\delta$) &0.57 $\pm$ 0.01 & 0.53 $\pm$ 0.03 & 0.61 $\pm$ 0.07 & 0.55 $\pm$ 0.04 & 0.50 $\pm$ 0.01 & 0.52 $\pm$ 0.01 & 0.51 $\pm$ 0.01 \\
 Pig & Only CB &0.58 $\pm$ 0.05 & 0.53 $\pm$ 0.01 & 0.56 $\pm$ 0.02 & 0.60 $\pm$ 0.06 & 0.51 $\pm$ 0.02 & 0.50 $\pm$ 0.01 & 0.52 $\pm$ 0.04 \\
 Pig & Only CB ($\mu$=0.25) &0.55 $\pm$ 0.01 & 0.52 $\pm$ 0.02 & 0.53 $\pm$ 0.02 & 0.55 $\pm$ 0.04 &   -   &   -   &   -   \\
 Pig & Only BC &  -   & 0.59 $\pm$ 0.03 & 0.57 $\pm$ 0.02 & 0.52 $\pm$ 0.01 &   -   &   -   &   -   \\
 Plankton & \spaplus (ours) &0.26 $\pm$ 0.01 & 0.23 $\pm$ 0.01 & 0.23 $\pm$ 0.01 & 0.22 $\pm$ 0.01 & 0.22 $\pm$ 0.01 & 0.22 $\pm$ 0.01 & 0.22 $\pm$ 0.01 \\
 Plankton & \spaplus (+ GT $\delta$) &0.26 $\pm$ 0.02 & 0.27 $\pm$ 0.01 & 0.27 $\pm$ 0.01 & 0.23 $\pm$ 0.01 & 0.21 $\pm$ 0.01 & 0.20 $\pm$ 0.02 & 0.20 $\pm$ 0.01 \\
 Plankton & Only CB &0.26 $\pm$ 0.01 & 0.23 $\pm$ 0.01 & 0.23 $\pm$ 0.01 & 0.22 $\pm$ 0.01 & 0.22 $\pm$ 0.01 & 0.22 $\pm$ 0.01 & 0.22 $\pm$ 0.01 \\
 Plankton & Only CB ($\mu$=0.25) &0.28 $\pm$ 0.02 & 0.25 $\pm$ 0.01 & 0.26 $\pm$ 0.02 & 0.26 $\pm$ 0.01 &   -   &   -   &   -   \\
 Plankton & Only BC &  -   & 0.28 $\pm$ 0.02 & 0.25 $\pm$ 0.01 & 0.24 $\pm$ 0.01 &   -   &   -   &   -   \\
 QualityMRI & \spaplus (ours) &0.24 $\pm$ 0.09 & 0.12 $\pm$ 0.03 & 0.11 $\pm$ 0.07 & 0.11 $\pm$ 0.05 & 0.10 $\pm$ 0.04 & 0.12 $\pm$ 0.04 & 0.16 $\pm$ 0.04 \\
 QualityMRI & \spaplus (+ GT $\delta$) &0.18 $\pm$ 0.10 & 0.18 $\pm$ 0.13 & 0.24 $\pm$ 0.08 & 0.11 $\pm$ 0.02 & 0.20 $\pm$ 0.05 & 0.24 $\pm$ 0.03 & 0.14 $\pm$ 0.05 \\
 QualityMRI & Only CB &0.20 $\pm$ 0.10 & 0.22 $\pm$ 0.02 & 0.15 $\pm$ 0.04 & 0.18 $\pm$ 0.10 & 0.15 $\pm$ 0.02 & 0.15 $\pm$ 0.09 & 0.16 $\pm$ 0.07 \\
 QualityMRI & Only CB ($\mu$=0.25) &0.11 $\pm$ 0.03 & 0.14 $\pm$ 0.05 & 0.07 $\pm$ 0.01 & 0.11 $\pm$ 0.05 &   -   &   -   &   -   \\
 QualityMRI & Only BC &  -   & 0.27 $\pm$ 0.18 & 0.27 $\pm$ 0.18 & 0.18 $\pm$ 0.14 &   -   &   -   &   -   \\
 Synthetic & \spaplus (ours) &0.08 $\pm$ 0.01 & 0.07 $\pm$ 0.01 & 0.08 $\pm$ 0.00 & 0.08 $\pm$ 0.00 & 0.08 $\pm$ 0.00 & 0.07 $\pm$ 0.01 & 0.07 $\pm$ 0.00 \\
 Synthetic & \spaplus (+ GT $\delta$) &0.08 $\pm$ 0.01 & 0.08 $\pm$ 0.01 & 0.08 $\pm$ 0.01 & 0.08 $\pm$ 0.00 & 0.08 $\pm$ 0.00 & 0.07 $\pm$ 0.01 & 0.08 $\pm$ 0.01 \\
 Synthetic & Only CB &0.08 $\pm$ 0.00 & 0.09 $\pm$ 0.01 & 0.08 $\pm$ 0.01 & 0.08 $\pm$ 0.00 & 0.08 $\pm$ 0.01 & 0.09 $\pm$ 0.02 & 0.09 $\pm$ 0.01 \\
 Synthetic & Only CB ($\mu$=0.25) &0.17 $\pm$ 0.01 & 0.16 $\pm$ 0.01 & 0.17 $\pm$ 0.01 & 0.18 $\pm$ 0.01 &   -   &   -   &   -   \\
 Synthetic & Only BC &  -   & 0.06 $\pm$ 0.00 & 0.05 $\pm$ 0.00 & 0.04 $\pm$ 0.00 &   -   &   -   &   -   \\
 Treeversity\#1 & \spaplus (ours) &0.39 $\pm$ 0.02 & 0.37 $\pm$ 0.01 & 0.37 $\pm$ 0.02 & 0.35 $\pm$ 0.01 & 0.35 $\pm$ 0.01 & 0.35 $\pm$ 0.02 & 0.35 $\pm$ 0.01 \\
 Treeversity\#1 & \spaplus (+ GT $\delta$) &0.39 $\pm$ 0.01 & 0.37 $\pm$ 0.01 & 0.37 $\pm$ 0.02 & 0.35 $\pm$ 0.01 & 0.36 $\pm$ 0.00 & 0.35 $\pm$ 0.01 & 0.36 $\pm$ 0.02 \\
 Treeversity\#1 & Only CB &0.40 $\pm$ 0.00 & 0.37 $\pm$ 0.01 & 0.36 $\pm$ 0.01 & 0.37 $\pm$ 0.02 & 0.36 $\pm$ 0.01 & 0.36 $\pm$ 0.01 & 0.36 $\pm$ 0.01 \\
 Treeversity\#1 & Only CB ($\mu$=0.25) &0.43 $\pm$ 0.01 & 0.41 $\pm$ 0.01 & 0.41 $\pm$ 0.01 & 0.40 $\pm$ 0.01 &   -   &   -   &   -   \\
 Treeversity\#1 & Only BC &  -   & 0.37 $\pm$ 0.02 & 0.37 $\pm$ 0.01 & 0.36 $\pm$ 0.01 &   -   &   -   &   -   \\
 Treeversity\#6 & \spaplus (ours) &0.47 $\pm$ 0.01 & 0.37 $\pm$ 0.02 & 0.34 $\pm$ 0.02 & 0.33 $\pm$ 0.01 & 0.30 $\pm$ 0.01 & 0.30 $\pm$ 0.01 & 0.28 $\pm$ 0.00 \\
 Treeversity\#6 & \spaplus (+ GT $\delta$) &0.47 $\pm$ 0.02 & 0.40 $\pm$ 0.01 & 0.35 $\pm$ 0.00 & 0.33 $\pm$ 0.01 & 0.31 $\pm$ 0.02 & 0.30 $\pm$ 0.00 & 0.30 $\pm$ 0.01 \\
 Treeversity\#6 & Only CB &0.47 $\pm$ 0.02 & 0.37 $\pm$ 0.00 & 0.36 $\pm$ 0.01 & 0.32 $\pm$ 0.00 & 0.31 $\pm$ 0.01 & 0.30 $\pm$ 0.00 & 0.30 $\pm$ 0.01 \\
 Treeversity\#6 & Only CB ($\mu$=0.25) &0.48 $\pm$ 0.01 & 0.45 $\pm$ 0.01 & 0.42 $\pm$ 0.01 & 0.41 $\pm$ 0.01 &   -   &   -   &   -   \\
 Treeversity\#6 & Only BC &  -   & 0.46 $\pm$ 0.03 & 0.42 $\pm$ 0.01 & 0.33 $\pm$ 0.02 &   -   &   -   &   -   \\
 Turkey & \spaplus (ours) &0.27 $\pm$ 0.00 & 0.25 $\pm$ 0.01 & 0.23 $\pm$ 0.02 & 0.22 $\pm$ 0.02 & 0.28 $\pm$ 0.10 & 0.20 $\pm$ 0.02 & 0.19 $\pm$ 0.01 \\
 Turkey & \spaplus (+ GT $\delta$) &0.29 $\pm$ 0.04 & 0.24 $\pm$ 0.01 & 0.20 $\pm$ 0.01 & 0.22 $\pm$ 0.03 & 0.20 $\pm$ 0.02 & 0.23 $\pm$ 0.05 & 0.19 $\pm$ 0.01 \\
 Turkey & Only CB &0.33 $\pm$ 0.07 & 0.29 $\pm$ 0.07 & 0.26 $\pm$ 0.06 & 0.22 $\pm$ 0.02 & 0.20 $\pm$ 0.01 & 0.21 $\pm$ 0.03 & 0.20 $\pm$ 0.02 \\
 Turkey & Only CB ($\mu$=0.25) &0.32 $\pm$ 0.02 & 0.26 $\pm$ 0.03 & 0.35 $\pm$ 0.12 & 0.24 $\pm$ 0.01 &   -   &   -   &   -   \\
 Turkey & Only BC &  -   & 0.24 $\pm$ 0.01 & 0.23 $\pm$ 0.05 & 0.23 $\pm$ 0.01 &   -   &   -   &   -   \\

 

			
			
		\end{tabular}
	}
		
\end{table*}
}

\newcommand{\tblBenchmarkAblationSecondPart}{
\begin{table*}[tb]
	\caption{
		Benchmark results ablation study,   metric: $\hat{KL}$ $\pm$ STD, columns are the number of annotations used
	}
	\label{tbl:BenchmarkAblationSecondPart}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{l c c c c c c c c c c c c c c c c}
			\toprule
			
		dataset & method & 1 & 3 & 5 & 10 & 20 & 50 & 100 \\

  \midrule 
  

Benthic & \spaplus (ours) &1.05 $\pm$ 0.03 & 0.51 $\pm$ 0.01 & 0.31 $\pm$ 0.01 & 0.20 $\pm$ 0.00 & 0.16 $\pm$ 0.00 & 0.13 $\pm$ 0.00 & 0.12 $\pm$ 0.00 \\
 Benthic & \spaplus (+ GT $\delta$) &1.05 $\pm$ 0.03 & 0.58 $\pm$ 0.00 & 0.39 $\pm$ 0.01 & 0.20 $\pm$ 0.00 & 0.11 $\pm$ 0.01 & 0.07 $\pm$ 0.00 & 0.05 $\pm$ 0.00 \\
 Benthic & Only CB &1.05 $\pm$ 0.03 & 0.52 $\pm$ 0.01 & 0.32 $\pm$ 0.01 & 0.22 $\pm$ 0.00 & 0.18 $\pm$ 0.00 & 0.16 $\pm$ 0.00 & 0.15 $\pm$ 0.00 \\
 Benthic & Only CB ($\mu$=0.25) &0.88 $\pm$ 0.03 & 0.55 $\pm$ 0.01 & 0.41 $\pm$ 0.01 & 0.35 $\pm$ 0.01 &   -   &   -   &   -   \\
 Benthic & Only BC &  -   & 1.43 $\pm$ 0.04 & 0.88 $\pm$ 0.03 & 0.35 $\pm$ 0.02 &   -   &   -   &   -   \\
 CIFAR10H & \spaplus (ours) &0.52 $\pm$ 0.03 & 0.17 $\pm$ 0.01 & 0.13 $\pm$ 0.00 & 0.10 $\pm$ 0.00 & 0.07 $\pm$ 0.00 & 0.04 $\pm$ 0.00 & 0.03 $\pm$ 0.00 \\
 CIFAR10H & \spaplus (+ GT $\delta$) &0.52 $\pm$ 0.03 & 0.16 $\pm$ 0.00 & 0.13 $\pm$ 0.00 & 0.09 $\pm$ 0.00 & 0.06 $\pm$ 0.00 & 0.03 $\pm$ 0.00 & 0.02 $\pm$ 0.00 \\
 CIFAR10H & Only CB &0.52 $\pm$ 0.03 & 0.17 $\pm$ 0.01 & 0.13 $\pm$ 0.00 & 0.09 $\pm$ 0.00 & 0.06 $\pm$ 0.00 & 0.03 $\pm$ 0.00 & 0.02 $\pm$ 0.00 \\
 CIFAR10H & Only CB ($\mu$=0.25) &0.49 $\pm$ 0.03 & 0.17 $\pm$ 0.01 & 0.13 $\pm$ 0.00 & 0.11 $\pm$ 0.00 &   -   &   -   &   -   \\
 CIFAR10H & Only BC &  -   & 0.29 $\pm$ 0.01 & 0.22 $\pm$ 0.00 & 0.15 $\pm$ 0.00 &   -   &   -   &   -   \\
 MiceBone & \spaplus (ours) &0.61 $\pm$ 0.02 & 0.28 $\pm$ 0.00 & 0.21 $\pm$ 0.01 & 0.14 $\pm$ 0.00 & 0.11 $\pm$ 0.01 & 0.09 $\pm$ 0.00 & 0.09 $\pm$ 0.01 \\
 MiceBone & \spaplus (+ GT $\delta$) &0.61 $\pm$ 0.02 & 0.34 $\pm$ 0.01 & 0.24 $\pm$ 0.02 & 0.13 $\pm$ 0.01 & 0.08 $\pm$ 0.00 & 0.05 $\pm$ 0.00 & 0.04 $\pm$ 0.00 \\
 MiceBone & Only CB &0.61 $\pm$ 0.02 & 0.28 $\pm$ 0.00 & 0.21 $\pm$ 0.01 & 0.15 $\pm$ 0.01 & 0.13 $\pm$ 0.01 & 0.11 $\pm$ 0.01 & 0.11 $\pm$ 0.01 \\
 MiceBone & Only CB ($\mu$=0.25) &0.40 $\pm$ 0.02 & 0.26 $\pm$ 0.01 & 0.24 $\pm$ 0.01 & 0.22 $\pm$ 0.01 &   -   &   -   &   -   \\
 MiceBone & Only BC &  -   & 1.39 $\pm$ 0.07 & 0.91 $\pm$ 0.04 & 0.40 $\pm$ 0.02 &   -   &   -   &   -   \\
 Pig & \spaplus (ours) &0.97 $\pm$ 0.03 & 0.44 $\pm$ 0.01 & 0.30 $\pm$ 0.01 & 0.19 $\pm$ 0.01 & 0.13 $\pm$ 0.00 & 0.10 $\pm$ 0.00 & 0.09 $\pm$ 0.00 \\
 Pig & \spaplus (+ GT $\delta$) &0.97 $\pm$ 0.03 & 0.48 $\pm$ 0.02 & 0.33 $\pm$ 0.00 & 0.19 $\pm$ 0.01 & 0.12 $\pm$ 0.00 & 0.07 $\pm$ 0.00 & 0.06 $\pm$ 0.00 \\
 Pig & Only CB &0.97 $\pm$ 0.03 & 0.44 $\pm$ 0.01 & 0.31 $\pm$ 0.01 & 0.20 $\pm$ 0.01 & 0.16 $\pm$ 0.01 & 0.13 $\pm$ 0.01 & 0.12 $\pm$ 0.00 \\
 Pig & Only CB ($\mu$=0.25) &0.57 $\pm$ 0.01 & 0.38 $\pm$ 0.00 & 0.33 $\pm$ 0.01 & 0.29 $\pm$ 0.01 &   -   &   -   &   -   \\
 Pig & Only BC &  -   & 2.02 $\pm$ 0.05 & 1.38 $\pm$ 0.02 & 0.56 $\pm$ 0.02 &   -   &   -   &   -   \\
 Plankton & \spaplus (ours) &0.59 $\pm$ 0.02 & 0.35 $\pm$ 0.03 & 0.29 $\pm$ 0.01 & 0.22 $\pm$ 0.01 & 0.16 $\pm$ 0.01 & 0.13 $\pm$ 0.00 & 0.12 $\pm$ 0.00 \\
 Plankton & \spaplus (+ GT $\delta$) &0.59 $\pm$ 0.02 & 0.50 $\pm$ 0.01 & 0.38 $\pm$ 0.02 & 0.21 $\pm$ 0.01 & 0.12 $\pm$ 0.01 & 0.06 $\pm$ 0.00 & 0.04 $\pm$ 0.00 \\
 Plankton & Only CB &0.59 $\pm$ 0.02 & 0.35 $\pm$ 0.03 & 0.29 $\pm$ 0.01 & 0.22 $\pm$ 0.01 & 0.16 $\pm$ 0.01 & 0.13 $\pm$ 0.00 & 0.12 $\pm$ 0.00 \\
 Plankton & Only CB ($\mu$=0.25) &0.54 $\pm$ 0.02 & 0.35 $\pm$ 0.03 & 0.32 $\pm$ 0.01 & 0.28 $\pm$ 0.01 &   -   &   -   &   -   \\
 Plankton & Only BC &  -   & 0.79 $\pm$ 0.06 & 0.68 $\pm$ 0.05 & 0.36 $\pm$ 0.02 &   -   &   -   &   -   \\
 QualityMRI & \spaplus (ours) &0.54 $\pm$ 0.06 & 0.16 $\pm$ 0.02 & 0.09 $\pm$ 0.02 & 0.05 $\pm$ 0.01 & 0.03 $\pm$ 0.01 & 0.02 $\pm$ 0.00 & 0.01 $\pm$ 0.00 \\
 QualityMRI & \spaplus (+ GT $\delta$) &0.54 $\pm$ 0.06 & 0.14 $\pm$ 0.02 & 0.10 $\pm$ 0.01 & 0.05 $\pm$ 0.00 & 0.02 $\pm$ 0.01 & 0.01 $\pm$ 0.00 & 0.01 $\pm$ 0.00 \\
 QualityMRI & Only CB &0.54 $\pm$ 0.06 & 0.15 $\pm$ 0.02 & 0.07 $\pm$ 0.02 & 0.04 $\pm$ 0.01 & 0.02 $\pm$ 0.01 & 0.01 $\pm$ 0.00 & 0.01 $\pm$ 0.00 \\
 QualityMRI & Only CB ($\mu$=0.25) &0.21 $\pm$ 0.03 & 0.09 $\pm$ 0.01 & 0.06 $\pm$ 0.01 & 0.06 $\pm$ 0.01 &   -   &   -   &   -   \\
 QualityMRI & Only BC &  -   & 1.06 $\pm$ 0.18 & 0.42 $\pm$ 0.10 & 0.10 $\pm$ 0.02 &   -   &   -   &   -   \\
 Synthetic & \spaplus (ours) &0.90 $\pm$ 0.01 & 0.44 $\pm$ 0.00 & 0.32 $\pm$ 0.00 & 0.19 $\pm$ 0.00 & 0.12 $\pm$ 0.00 & 0.08 $\pm$ 0.00 & 0.07 $\pm$ 0.00 \\
 Synthetic & \spaplus (+ GT $\delta$) &0.90 $\pm$ 0.01 & 0.49 $\pm$ 0.01 & 0.38 $\pm$ 0.00 & 0.21 $\pm$ 0.01 & 0.13 $\pm$ 0.00 & 0.07 $\pm$ 0.00 & 0.06 $\pm$ 0.00 \\
 Synthetic & Only CB &0.90 $\pm$ 0.01 & 0.42 $\pm$ 0.00 & 0.30 $\pm$ 0.01 & 0.19 $\pm$ 0.00 & 0.13 $\pm$ 0.00 & 0.09 $\pm$ 0.00 & 0.08 $\pm$ 0.00 \\
 Synthetic & Only CB ($\mu$=0.25) &0.64 $\pm$ 0.01 & 0.39 $\pm$ 0.00 & 0.34 $\pm$ 0.01 & 0.27 $\pm$ 0.00 &   -   &   -   &   -   \\
 Synthetic & Only BC &  -   & 1.52 $\pm$ 0.01 & 1.16 $\pm$ 0.01 & 0.54 $\pm$ 0.01 &   -   &   -   &   -   \\
 Treeversity\#1 & \spaplus (ours) &0.76 $\pm$ 0.04 & 0.27 $\pm$ 0.02 & 0.20 $\pm$ 0.01 & 0.12 $\pm$ 0.01 & 0.08 $\pm$ 0.00 & 0.06 $\pm$ 0.00 & 0.05 $\pm$ 0.00 \\
 Treeversity\#1 & \spaplus (+ GT $\delta$) &0.76 $\pm$ 0.04 & 0.27 $\pm$ 0.02 & 0.20 $\pm$ 0.01 & 0.12 $\pm$ 0.01 & 0.08 $\pm$ 0.00 & 0.05 $\pm$ 0.00 & 0.04 $\pm$ 0.00 \\
 Treeversity\#1 & Only CB &0.76 $\pm$ 0.04 & 0.27 $\pm$ 0.02 & 0.20 $\pm$ 0.01 & 0.12 $\pm$ 0.01 & 0.09 $\pm$ 0.00 & 0.07 $\pm$ 0.00 & 0.06 $\pm$ 0.00 \\
 Treeversity\#1 & Only CB ($\mu$=0.25) &0.64 $\pm$ 0.03 & 0.30 $\pm$ 0.01 & 0.25 $\pm$ 0.00 & 0.20 $\pm$ 0.00 &   -   &   -   &   -   \\
 Treeversity\#1 & Only BC &  -   & 0.68 $\pm$ 0.04 & 0.50 $\pm$ 0.02 & 0.23 $\pm$ 0.01 &   -   &   -   &   -   \\
 Treeversity\#6 & \spaplus (ours) &1.11 $\pm$ 0.03 & 0.46 $\pm$ 0.01 & 0.30 $\pm$ 0.01 & 0.18 $\pm$ 0.01 & 0.11 $\pm$ 0.00 & 0.07 $\pm$ 0.00 & 0.06 $\pm$ 0.00 \\
 Treeversity\#6 & \spaplus (+ GT $\delta$) &1.11 $\pm$ 0.03 & 0.50 $\pm$ 0.01 & 0.36 $\pm$ 0.01 & 0.20 $\pm$ 0.00 & 0.12 $\pm$ 0.00 & 0.07 $\pm$ 0.00 & 0.06 $\pm$ 0.00 \\
 Treeversity\#6 & Only CB &1.11 $\pm$ 0.03 & 0.45 $\pm$ 0.01 & 0.29 $\pm$ 0.00 & 0.17 $\pm$ 0.00 & 0.12 $\pm$ 0.00 & 0.09 $\pm$ 0.00 & 0.08 $\pm$ 0.00 \\
 Treeversity\#6 & Only CB ($\mu$=0.25) &0.74 $\pm$ 0.02 & 0.42 $\pm$ 0.01 & 0.33 $\pm$ 0.01 & 0.27 $\pm$ 0.01 &   -   &   -   &   -   \\
 Treeversity\#6 & Only BC &  -   & 1.85 $\pm$ 0.01 & 1.38 $\pm$ 0.03 & 0.61 $\pm$ 0.02 &   -   &   -   &   -   \\
 Turkey & \spaplus (ours) &0.38 $\pm$ 0.03 & 0.14 $\pm$ 0.01 & 0.10 $\pm$ 0.01 & 0.06 $\pm$ 0.00 & 0.04 $\pm$ 0.00 & 0.03 $\pm$ 0.00 & 0.02 $\pm$ 0.00 \\
 Turkey & \spaplus (+ GT $\delta$) &0.38 $\pm$ 0.03 & 0.14 $\pm$ 0.01 & 0.10 $\pm$ 0.01 & 0.06 $\pm$ 0.00 & 0.04 $\pm$ 0.00 & 0.03 $\pm$ 0.00 & 0.02 $\pm$ 0.00 \\
 Turkey & Only CB &0.38 $\pm$ 0.03 & 0.14 $\pm$ 0.01 & 0.10 $\pm$ 0.01 & 0.06 $\pm$ 0.01 & 0.04 $\pm$ 0.00 & 0.03 $\pm$ 0.00 & 0.03 $\pm$ 0.00 \\
 Turkey & Only CB ($\mu$=0.25) &0.27 $\pm$ 0.02 & 0.14 $\pm$ 0.01 & 0.12 $\pm$ 0.01 & 0.10 $\pm$ 0.01 &   -   &   -   &   -   \\
 Turkey & Only BC &  -   & 0.43 $\pm$ 0.03 & 0.28 $\pm$ 0.02 & 0.13 $\pm$ 0.01 &   -   &   -   &   -   \\



			
			
		\end{tabular}
	}
		
\end{table*}
}

\newcommand{\tblBenchmarkAblationThirdPart}{
\begin{table*}[tb]
	\caption{
		Benchmark results ablation study,   metric: $KL$ $\pm$ STD but evaluated on a transformer backbone, columns are the number of annotations used
	}
	\label{tbl:BenchmarkAblationThirdPart}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{l c c c c c c c c c c c c c c c c}
			\toprule
			
		dataset & method & 1 & 3 & 5 & 10 & 20 & 50 & 100 \\

\midrule

Benthic & \spaplus (+ GT $\delta$) &  -   & 0.50 $\pm$ 0.02 &   -   & 0.46 $\pm$ 0.01 &   -   &   -   & 0.43 $\pm$ 0.01 \\
 Benthic & Only CB &  -   & 0.47 $\pm$ 0.00 &   -   & 0.46 $\pm$ 0.02 &   -   &   -   & 0.45 $\pm$ 0.01 \\
 CIFAR10H & \spaplus (+ GT $\delta$) &  -   & 0.10 $\pm$ 0.00 &   -   & 0.10 $\pm$ 0.00 &   -   &   -   & 0.10 $\pm$ 0.00 \\
 CIFAR10H & Only CB &  -   & 0.10 $\pm$ 0.00 &   -   & 0.10 $\pm$ 0.00 &   -   &   -   & 0.10 $\pm$ 0.00 \\
 MiceBone & \spaplus (+ GT $\delta$) &  -   & 0.22 $\pm$ 0.02 &   -   & 0.19 $\pm$ 0.02 &   -   &   -   & 0.17 $\pm$ 0.02 \\
 MiceBone & Only CB &  -   & 0.21 $\pm$ 0.02 &   -   & 0.19 $\pm$ 0.01 &   -   &   -   & 0.19 $\pm$ 0.01 \\
 Pig & \spaplus (+ GT $\delta$) &  -   & 0.45 $\pm$ 0.01 &   -   & 0.38 $\pm$ 0.01 &   -   &   -   & 0.34 $\pm$ 0.01 \\
 Pig & Only CB &  -   & 0.44 $\pm$ 0.01 &   -   & 0.39 $\pm$ 0.01 &   -   &   -   & 0.36 $\pm$ 0.01 \\
 Plankton & \spaplus (+ GT $\delta$) &  -   & 0.22 $\pm$ 0.01 &   -   & 0.19 $\pm$ 0.01 &   -   &   -   & 0.16 $\pm$ 0.01 \\
 Plankton & Only CB &  -   & 0.19 $\pm$ 0.01 &   -   & 0.18 $\pm$ 0.01 &   -   &   -   & 0.18 $\pm$ 0.01 \\
 QualityMRI & \spaplus (+ GT $\delta$) &  -   & 0.05 $\pm$ 0.00 &   -   & 0.04 $\pm$ 0.00 &   -   &   -   & 0.05 $\pm$ 0.00 \\
 QualityMRI & Only CB &  -   & 0.06 $\pm$ 0.00 &   -   & 0.05 $\pm$ 0.01 &   -   &   -   & 0.05 $\pm$ 0.01 \\
 Synthetic & \spaplus (+ GT $\delta$) &  -   & 0.07 $\pm$ 0.00 &   -   & 0.06 $\pm$ 0.00 &   -   &   -   & 0.04 $\pm$ 0.00 \\
 Synthetic & Only CB &  -   & 0.08 $\pm$ 0.00 &   -   & 0.07 $\pm$ 0.00 &   -   &   -   & 0.07 $\pm$ 0.00 \\
 Treeversity\#1 & \spaplus (+ GT $\delta$) &  -   & 0.24 $\pm$ 0.01 &   -   & 0.21 $\pm$ 0.01 &   -   &   -   & 0.20 $\pm$ 0.01 \\
 Treeversity\#1 & Only CB &  -   & 0.24 $\pm$ 0.01 &   -   & 0.21 $\pm$ 0.01 &   -   &   -   & 0.21 $\pm$ 0.01 \\
 Treeversity\#6 & \spaplus (+ GT $\delta$) &  -   & 0.24 $\pm$ 0.01 &   -   & 0.18 $\pm$ 0.01 &   -   &   -   & 0.15 $\pm$ 0.00 \\
 Treeversity\#6 & Only CB &  -   & 0.24 $\pm$ 0.01 &   -   & 0.18 $\pm$ 0.01 &   -   &   -   & 0.16 $\pm$ 0.01 \\
 Turkey & \spaplus (+ GT $\delta$) &  -   & 0.18 $\pm$ 0.02 &   -   & 0.16 $\pm$ 0.01 &   -   &   -   & 0.16 $\pm$ 0.01 \\
 Turkey & Only CB &  -   & 0.18 $\pm$ 0.00 &   -   & 0.16 $\pm$ 0.01 &   -   &   -   & 0.16 $\pm$ 0.01 \\

			
			
		\end{tabular}
	}
		
\end{table*}
}


\newcommand{\tblBenchmarkAblationMedian}{
\begin{table}[tb]
	\caption{
		Benchmark results ablation study, first block of rows $KL$ result on normal benchmark, second block of rows $\hat{KL}$ on benchmark, last block of rows $KL$ results on benchmark but with ViT as backbone, all results are median aggregations across the datasets
	}
	\label{tbl:BenchmarkAblationMedian}
 \centering
	\resizebox{\linewidth}{!}{
		\begin{tabular}{l c c c c c c c c c c c c c c c c c c c c c}
			\toprule
			
		method &&  1 && 3 && 5 && 10 && 20 && 50 && 100 \\
  \midrule
\spaplus (ours) &&0.29 $\pm$ 0.02 && 0.28 $\pm$ 0.01 && 0.26 $\pm$ 0.02 && 0.25 $\pm$ 0.01 && 0.27 $\pm$ 0.02 && 0.25 $\pm$ 0.02 && 0.24 $\pm$ 0.01 \\
 \spaplus (+ GT $\delta$) &&0.30 $\pm$ 0.02 && 0.28 $\pm$ 0.01 && 0.27 $\pm$ 0.01 && 0.25 $\pm$ 0.02 && 0.24 $\pm$ 0.01 && 0.24 $\pm$ 0.01 && 0.24 $\pm$ 0.01 \\
 Only CB &&0.34 $\pm$ 0.03 && 0.28 $\pm$ 0.01 && 0.27 $\pm$ 0.01 && 0.25 $\pm$ 0.02 && 0.25 $\pm$ 0.01 && 0.25 $\pm$ 0.02 && 0.25 $\pm$ 0.02 \\
 Only CB ($\mu$=0.25) &&0.33 $\pm$ 0.02 && 0.28 $\pm$ 0.01 && 0.33 $\pm$ 0.02 && 0.29 $\pm$ 0.01 &&   -   &&   -   &&   -   \\
 Only BC &&  -   && 0.30 $\pm$ 0.02 && 0.29 $\pm$ 0.02 && 0.26 $\pm$ 0.02 &&   -   &&   -   &&   -   \\






\midrule

\spaplus (ours) &&0.68 $\pm$ 0.03 && 0.32 $\pm$ 0.01 && 0.25 $\pm$ 0.01 && 0.16 $\pm$ 0.00 && 0.11 $\pm$ 0.00 && 0.08 $\pm$ 0.00 && 0.07 $\pm$ 0.00 \\
 \spaplus (+ GT $\delta$) &&0.68 $\pm$ 0.03 && 0.41 $\pm$ 0.01 && 0.29 $\pm$ 0.01 && 0.16 $\pm$ 0.00 && 0.10 $\pm$ 0.00 && 0.05 $\pm$ 0.00 && 0.04 $\pm$ 0.00 \\
 Only CB &&0.68 $\pm$ 0.03 && 0.32 $\pm$ 0.01 && 0.25 $\pm$ 0.01 && 0.16 $\pm$ 0.01 && 0.12 $\pm$ 0.00 && 0.09 $\pm$ 0.00 && 0.08 $\pm$ 0.00 \\
 Only CB ($\mu$=0.25) &&0.55 $\pm$ 0.02 && 0.33 $\pm$ 0.01 && 0.29 $\pm$ 0.01 && 0.24 $\pm$ 0.01 &&   -   &&   -   &&   -   \\
 Only BC &&  -   && 1.22 $\pm$ 0.04 && 0.78 $\pm$ 0.02 && 0.36 $\pm$ 0.02 &&   -   &&   -   &&   -   \\




 \midrule

\spaplus (+ GT $\delta$) &&  -   && 0.22 $\pm$ 0.01 &&   -   && 0.18 $\pm$ 0.01 &&   -   &&   -   && 0.16 $\pm$ 0.01 \\
 Only CB &&  -   && 0.20 $\pm$ 0.01 &&   -   && 0.18 $\pm$ 0.01 &&   -   &&   -   && 0.17 $\pm$ 0.01 \\

			
			
		\end{tabular}
	}
		
\end{table}
}

\newcommand{\tblBenchmarkAblationMean}{
\begin{table}[tb]
	\caption{
		Benchmark results ablation study, first block of rows $KL$ result on normal benchmark, second block of rows $\hat{KL}$ on benchmark, last block of rows $KL$ results on benchmark but with ViT as backbone, all results are mean aggregations across the datasets
	}
	\label{tbl:BenchmarkAblationMean}
 \centering
	\resizebox{\linewidth}{!}{
		\begin{tabular}{l c c c c c c c c c c c c c c c c}
			\toprule
			
		method &  1 & 3 & 5 & 10 & 20 & 50 & 100 \\
  \midrule

\spaplus (ours) &0.37 $\pm$ 0.02 & 0.33 $\pm$ 0.02 & 0.32 $\pm$ 0.03 & 0.30 $\pm$ 0.02 & 0.31 $\pm$ 0.03 & 0.29 $\pm$ 0.02 & 0.29 $\pm$ 0.02 \\
 \spaplus (+ GT $\delta$) &0.36 $\pm$ 0.03 & 0.34 $\pm$ 0.02 & 0.34 $\pm$ 0.03 & 0.30 $\pm$ 0.02 & 0.30 $\pm$ 0.02 & 0.30 $\pm$ 0.02 & 0.29 $\pm$ 0.02 \\
 Only CB &0.37 $\pm$ 0.04 & 0.34 $\pm$ 0.02 & 0.32 $\pm$ 0.02 & 0.32 $\pm$ 0.03 & 0.30 $\pm$ 0.01 & 0.30 $\pm$ 0.02 & 0.30 $\pm$ 0.02 \\
 Only CB ($\mu$=0.25) &0.38 $\pm$ 0.02 & 0.35 $\pm$ 0.02 & 0.35 $\pm$ 0.03 & 0.34 $\pm$ 0.02 &   -   &   -   &   -   \\
 Only BC &  -   & 0.38 $\pm$ 0.05 & 0.35 $\pm$ 0.04 & 0.31 $\pm$ 0.03 &   -   &   -   &   -   \\





\midrule


 \spaplus (ours) &0.74 $\pm$ 0.03 & 0.32 $\pm$ 0.01 & 0.22 $\pm$ 0.01 & 0.14 $\pm$ 0.01 & 0.10 $\pm$ 0.00 & 0.07 $\pm$ 0.00 & 0.07 $\pm$ 0.00 \\
 \spaplus (+ GT $\delta$) &0.74 $\pm$ 0.03 & 0.36 $\pm$ 0.01 & 0.26 $\pm$ 0.01 & 0.14 $\pm$ 0.00 & 0.09 $\pm$ 0.00 & 0.05 $\pm$ 0.00 & 0.04 $\pm$ 0.00 \\
 Only CB &0.74 $\pm$ 0.03 & 0.32 $\pm$ 0.01 & 0.22 $\pm$ 0.01 & 0.15 $\pm$ 0.01 & 0.11 $\pm$ 0.00 & 0.09 $\pm$ 0.00 & 0.08 $\pm$ 0.00 \\
 Only CB ($\mu$=0.25) &0.54 $\pm$ 0.02 & 0.31 $\pm$ 0.01 & 0.25 $\pm$ 0.01 & 0.21 $\pm$ 0.01 &   -   &   -   &   -   \\
 Only BC &  -   & 1.15 $\pm$ 0.05 & 0.78 $\pm$ 0.03 & 0.34 $\pm$ 0.02 &   -   &   -   &   -   \\






 \midrule

\spaplus (+ GT $\delta$) &  -   & 0.23 $\pm$ 0.01 &   -   & 0.20 $\pm$ 0.01 &   -   &   -   & 0.18 $\pm$ 0.01 \\
 Only CB &  -   & 0.22 $\pm$ 0.01 &   -   & 0.20 $\pm$ 0.01 &   -   &   -   & 0.19 $\pm$ 0.01 \\



			
			
		\end{tabular}
	}
		
\end{table}
}

\newcommand{\tblBenchmarkAblationMedianShort}{
\begin{table}[tb]
	\caption{
		Benchmark results ablation study, first block of rows $KL$ result on normal benchmark, second block of rows $\hat{KL}$ on benchmark, last block of rows $KL$ results on benchmark but with ViT as backbone, all results are median aggregations across the datasets
	}
	\label{tbl:BenchmarkAblationMedianShort}
 \centering
	\resizebox{\linewidth}{!}{
		\begin{tabular}{p{4cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm}}
			\toprule
			
		method &  1 & 3 & 5 & 10 & 20 & 50 & 100 \\
  \midrule
\spaplus (ours) &0.29  & 0.28 & 0.26  & 0.25  & 0.27  & 0.25  & 0.24  \\
 \spaplus (+ GT $\delta$) &0.30  & 0.28 & 0.27& 0.25  & 0.24  & 0.24  & 0.24 \\
 Only CB &0.34 & 0.28 & 0.27 & 0.25 & 0.25  & 0.25 & 0.25  \\
 Only CB ($\mu$=0.25) &0.33  & 0.28 & 0.33  & 0.29  &   -   &   -   &   -   \\
 Only BC &  -   & 0.30  & 0.29  & 0.26 &   -   &   -   &   -   \\






\midrule

\spaplus (ours) &0.68  & 0.32  & 0.25  & 0.16  & 0.11  & 0.08  & 0.07  \\
 \spaplus (+ GT $\delta$) &0.68  & 0.41 & 0.29  & 0.16  & 0.10 & 0.05 & 0.04 \\
 Only CB &0.68  & 0.32  & 0.25  & 0.16 & 0.12  & 0.09  & 0.08  \\
 Only CB ($\mu$=0.25) &0.55  & 0.33  & 0.29  & 0.24 &   -   &   -   &   -   \\
 Only BC &  -   & 1.22 & 0.78 & 0.36 &   -   &   -   &   -   \\




 \midrule

\spaplus (+ GT $\delta$) &  -   & 0.22 &   -   & 0.18 &   -   &   -   & 0.16 \\
 Only CB &  -   & 0.20  &   -   & 0.18  &   -   &   -   & 0.17 \\

			
			
		\end{tabular}
	}
		
\end{table}
}
